An Exponential Time Parameterized Algorithm for Planar Disjoint Paths

In the Disjoint Paths problem, the input is an undirected graph $G$ on $n$ vertices and a set of $k$ vertex pairs, $\{s_i,t_i\}_{i=1}^k$, and the task is to find $k$ pairwise vertex-disjoint paths connecting $s_i$ to $t_i$. The problem was shown to have an $f(k)n^3$ algorithm by Robertson and Seymour. In modern terminology, this means that Disjoint Paths is fixed parameter tractable (FPT), parameterized by the number of vertex pairs. This algorithm is the cornerstone of the entire graph minor theory, and a vital ingredient in the $g(k)n^3$ algorithm for Minor Testing (given two undirected graphs, $G$ and $H$ on $n$ and $k$ vertices, respectively, the objective is to check whether $G$ contains $H$ as a minor). All we know about $f$ and $g$ is that these are computable functions. Thus, a challenging open problem in graph algorithms is to devise an algorithm for Disjoint Paths where $f$ is single exponential. That is, $f$ is of the form $2^{{\sf poly}(k)}$. The algorithm of Robertson and Seymour relies on topology and essentially reduces the problem to surface-embedded graphs. Thus, the first major obstacle that has to be overcome in order to get an algorithm with a single exponential running time for Disjoint Paths and {\sf Minor Testing} on general graphs is to solve Disjoint Paths in single exponential time on surface-embedded graphs and in particular on planar graphs. Even when the inputs to Disjoint Paths are restricted to planar graphs, a case called the Planar Disjoint Paths problem, the best known algorithm has running time $2^{2^{O(k)}}n^2$. In this paper, we make the first step towards our quest for designing a single exponential time algorithm for Disjoint Paths by giving a $2^{O(k^2)}n^{O(1)}$-time algorithm for Planar Disjoint Paths.

==> homologyPhases.tex <==
\subsection{Phase I: Eliminating Non-Spiraling Boring Sequences}

We begin pushing a flow onto a Steiner tree $R$ by pushing all boring non-spiraling sequences of its walk extraction. To this end, we need to identify which non-spiraling boring sequence is to be pushed. This is done in the following definition 
%(see Fig.~\hlg{FIG})
, based on the notion of $\RB(Q)$ in  Definition \ref{def:usefulSubwalkClosure}. Here, we assume that the parallel edges of $A(R)$ taken to construct $\RB(Q)$ are those indexed $1$. % (see Fig.~\hlg{FIG}). 
We use the same convention when referring to paths on $R$ using the notation $\pathT_R$.

\begin{definition}[{\bf Innermost Non-Spiral Boring Sequence}]\label{def:innermostNonspiralBoring}
Let $(D,S,T,g,k)$ be a nice instance of \dpdp. Let $R$ be a Steiner tree. Let $\phi: A(H_D)\rightarrow \RW(T)$ be a flow. Let $\{\stitch_{\phi,v}\}|_{v\in V(H_D)}$ be a stitching of $\phi$ such that $(\phi,\{\stitch_{\phi,v}\}|_{v\in V(H_D)})$ is non-cyclic and well-behaved. Let $\cal W$ be the walk extraction of $(\phi,\{\stitch_{\phi,v}\}|_{v\in V(H_D)})$. A non-spiraling boring sequence $Q\in\Seq(W)$ for some $W\in{\cal W}$ is {\em innermost} if it is not pushed and the strict interior of $\RB(Q)$ contains no arc that belongs to $(\bigcup_{W\in{\cal W}}A(W))\setminus A(R)$.\footnote{Note that even if the strict interior of $\RB(Q)$ contains no vertex that belongs to $\bigcup_{W\in{\cal W}}V(W)$, it may still contain arcs that belong to $(\bigcup_{W\in{\cal W}}A(W))\setminus A(R)$ (which may be boring sequences of walks in $\cal W$).}
\end{definition}

We show that if there exist non-spiraling boring sequences in our collection, then there exists at least one that is innermost.

\begin{lemma}\label{lem:innermostNonspiralBoringExists}
Let $(D,S,T,g,k)$ be a nice instance of \dpdp. Let $R$ be a Steiner tree. Let $\phi: A(H_D)\rightarrow \RW(T)$ be a flow. Let $\{\stitch_{\phi,v}\}|_{v\in V(H_D)}$ be a stitching of $\phi$ such that $(\phi,\{\stitch_{\phi,v}\}|_{v\in V(H_D)})$ is non-cyclic and well-behaved. Let $\cal W$ be the walk extraction of $(\phi,\{\stitch_{\phi,v}\}|_{v\in V(H_D)})$. If there exist non-spiraling non-pushed boring sequences in $\bigcup_{W\in{\cal W}}\Seq(W)$, then there exists an innermost non-spiraling boring sequence in $\bigcup_{W\in{\cal W}}\Seq(W)$.
\end{lemma}

\begin{proof}
    % These commands are defined only within this proof environment
    \newcommand{\VR}{V_{=1}(R) \cup V_{\geq 3}(R)}
    \newcommand{\W}{{\cal W}}
    \renewcommand{\st}{\stitch}
    %\hlb{TODO (PM): use well-behaved property to make proof easier}
    Consider a non-pushed non-spiraling boring sequence $Q \in \bigcup_{W \in \W} \Seq(W)$, and the cycle $\RB(Q)$. Observe that, as $Q$ is boring, $\Plunder(Q) = \emptyset$, and hence the two endpoints of $Q$ are internal vertices of the same maximal degree-2 path of $R$. Otherwise there will be a vertex in $\VR$ that either lies on $\RB(Q)$ or it's strict interior, contradicting the fact that $\Plunder(Q) = \emptyset$.
    Let us assume that $Q$ is chosen so that $I_Q$ contains the fewest vertices of $V(D)$
    
    Now consider any other sequence non-spiraling boring subwalk $P \in \bigcup_{W \in \W} \Seq(W)$ that is non-pushed and $P$ contains an arc $e$ that is in the strict interior of $I_Q$. Then by Observation~\ref{obs:SeqRBLaminar1}, $I_P \subset I_Q$ since the points on $e$ are excluded from $I_P$, but are present in $I_Q$. Then it follows that $P$ is contained in $\RB(Q)$ (Observation~\ref{obs:SeqRBLaminar2}), 
    and $I_P$ contains strictly fewer vertices of $V(R)$ than $I_Q$, since an endpoint of the arc $e$ must be excluded from $I_P$, but it is present in $I_Q$. But this contradicts the choice of $Q$.
    Hence there is no such sequence $P$.
    
    Now the only other non-pushed sequences in $\bigcup_{W\in{\cal W}}\Seq(W)$ may be spirals or interesting sequences, both of which have non empty plunder. Hence if an arc of such a sequence $P$ lies strictly within $I_Q$, then as before $I_P \subsetneq I_Q$. But then $\RB(P)$ is contained in $\RB(Q) \cup I_Q$, which contradicts that $\Plunder(P) \neq \emptyset$.
  
    Hence we conclude that there is no non-pushed sequence such that an arc of this sequence lies in the interior of $\RB(Q)$. Since any arc in $(\bigcup_{W\in{\cal W}}A(W))\setminus A(R)$ must lie on some non-pushed sequence in $\bigcup_{W\in{\cal W}} \Seq(W)$ it follows that no arc in $(\bigcup_{W\in{\cal W}}A(W))\setminus A(R)$ lies in the interior of $\RB(Q)$.
    Hence we conclude that $Q$ is the required non-spiraling non-pushed sequence in $\bigcup_{W\in{\cal W}}\Seq(W)$.
\end{proof}

Towards the definition of the elimination of the sequence we have just identified, we need the following definition. %(see Fig.~\hlg{FIG}).

\begin{definition}[{\bf Projection of Non-Spiral Boring Sequence}]\label{def:projectionNonspiralBoring}
Let $(D,S,T,g,k)$ be a nice instance of \dpdp. Let $R$ be a Steiner tree. Let $\phi: A(H_D)\rightarrow \RW(T)$ be a flow. Let $\{\stitch_{\phi,v}\}|_{v\in V(H_D)}$ be a stitching of $\phi$ such that $(\phi,\{\stitch_{\phi,v}\}|_{v\in V(H_D)})$ is shallow, non-cyclic and well-behaved. Let $\cal W$ be the walk extraction of $(\phi,\{\stitch_{\phi,v}\}|_{v\in V(H_D)})$. Let $Q\in\Seq(W)$ for some $W\in{\cal W}$ be a non-spiraling boring sequence. Then, the {\em projection of $Q$ with respect to $(\phi,\{\stitch_{\phi,v}\}|_{v\in V(H_D)})$}, denoted by $\Project(Q)$,\footnote{This notation will be used only when $(\phi,\{\stitch_{\phi,v}\}|_{v\in V(H_D)})$ is clear from context.} is the set of arcs in $\bigcup_{e\in A(R)\cap \RB(Q)}\Parallel(e)$ with the index 
\[b\cdot(|V(H_D)|-\dist(\phi,\{\stitch_{\phi,v}\}|_{v\in V(H_D)})+1),\] where $b\in\{-1,1\}$ is defined as follows.
\begin{itemize}
\item If the interior of $\RB(Q)$ contains edges in $A(R)$ indexed $-1$, then $b=-1$.
\item Otherwise, $b=1$.
\end{itemize}
\end{definition}

We now show how to eliminate the sequence. This will be done in two steps. In the first step, we define the flow that results from the elimination. % (see Fig.~\hlg{FIG}).

\begin{definition}[{\bf Flow-Component of Elimination of a Non-Spiral Boring Sequence}]\label{def:innermostNonspiralBoringElimination}
Let $(D,S,T,g,k)$ be a nice instance of \dpdp. Let $R$ be a Steiner tree. Let $\phi: A(H_D)\rightarrow \RW(T)$ be a flow. Let $\{\stitch_{\phi,v}\}|_{v\in V(H_D)}$ be a stitching of $\phi$ such that $(\phi,\{\stitch_{\phi,v}\}|_{v\in V(H_D)})$ is shallow, non-cyclic and well-behaved. Let $\cal W$ be the walk extraction of $(\phi,\{\stitch_{\phi,v}\}|_{v\in V(H_D)})$. Let $Q\in\Seq(W)$ for some $W\in{\cal W}$ be an innermost non-spiraling boring sequence. The {\em flow-component of the elimination of $Q$ in $(\phi,\{\stitch_{\phi,v}\}|_{v\in V(H_D)})$} is the function $\psi: A(D)\rightarrow \RW(T)$ defined as~follows.
\begin{itemize}
\item For every arc $e\in A(Q)$, define $\psi(e)=1$.
\item For every arc $e\in A(H_D)\setminus (A(Q)\cup \Project(Q))$, define $\psi(e)=\phi(e)$.
\item Let $x$ and $y$ be the endpoints of $Q$ such that $x$ is visited before $y$ when $W$ is traversed from its endpoint $s\in S$ to its endpoint $g(s)\in T$.\footnote{As $(\wl_{\phi},\{\stitch_{\phi,v}\}|_{v\in V(H_D)})$ is sensible (by Lemma \ref{lem:sensibleStitching}), the selection of these endpoints is valid.} Then, for every arc $e\in\Project(Q)$ with source $u$ and target $v$,
	\begin{itemize}
	\item if $\dist_R(x,u)<\dist_R(x,v)$,\footnote{Note that we measure the distance as the length of the shortest {\em undirected} path in $R$ between the two specified vertices.} then $\psi(e)=t$, and
	\item otherwise, $\psi(e)=t^{-1}$.
\end{itemize}
\end{itemize}
\end{definition}

First, we assert that the flow-component in Definition \ref{def:innermostNonspiralBoringElimination} is a flow homologous to its origin. To simplify the proof, we will utilize the following proposition.

\begin{proposition}[\cite{DBLP:journals/siamcomp/Schrijver94}]\label{prop:functionOnFlow}
Let $D$ be a directed plane graph. Let $\Sigma$ be an alphabet. Let $\phi,\psi: A(G)\rightarrow \RW(\Sigma)$ be homologous functions. If $\phi$ is a flow, then so is $\psi$.
\end{proposition}

Having this proposition at hand, we proceed with our analysis.

\begin{lemma}\label{lem:flowCompIsHomFlow}
Let $(D,S,T,g,k)$ be a nice instance of \dpdp. Let $R$ be a Steiner tree. Let $\phi: A(H_D)\rightarrow \RW(T)$ be a flow. Let $\{\stitch_{\phi,v}\}|_{v\in V(H_D)}$ be a stitching of $\phi$ such that $(\phi,\{\stitch_{\phi,v}\}|_{v\in V(H_D)})$ is shallow, non-cyclic and well-behaved. Let $\cal W$ be the walk extraction of $(\phi,\{\stitch_{\phi,v}\}|_{v\in V(H_D)})$. Let $Q\in\Seq(W)$ for some $W\in{\cal W}$ be an innermost non-spiraling boring sequence. Then, the flow-component $\psi$ of the elimination of $Q$ in $(\phi,\{\stitch_{\phi,v}\}|_{v\in V(H_D)})$ is a flow homologous to $\phi$.
\end{lemma}

\begin{proof}
Let $\cal F$ be the set of faces of $H_D$. In light of Proposition \ref{prop:functionOnFlow}, to prove the lemma, it suffices to show that there exists a function $f: {\cal F}\rightarrow \RW(\Sigma)$ such that {\em (i)} $f(F)=1$ for the outer face $F$ of $H_D$, and {\em (ii)} for every arc $e\in A(H_D)$, it holds that $f(F)^{-1}\cdot \phi(e)\cdot f(F')=\psi(e)$ where $F$ and $F'$ are the faces at the left-hand side and the right-hand side of $e$, respectively. We define a function $f: {\cal F}\rightarrow \RW(\Sigma)$ as follows. Let $C$ be the cycle that consists of $Q$ and $\Project(Q)$, and let $x$ and $y$ be the endpoints of $Q$ such that $x$ is visited before $y$ when $W$ is traversed from its endpoint $s\in S$ to its endpoint $t=g(s)\in T$. Then,
\begin{itemize}
\item for every face $F\in{\cal F}$ in the interior of $C$, define $f(F)=t$ if the interior of $C$ is to the left-hand side of $Q$ (when oriented from $x$ to $y$), and $f(F)=t^{-1}$ otherwise;
\item for every face $F\in{\cal F}$ in the exterior of $C$, define $f(F)=1$.
\end{itemize}
Since the outer face of $D$ is incident to a terminal, Condition {\em (i)} is clearly satisfied. Now, we turn to verify that Condition {\em (ii)} is satisfied. To this end, consider some arc $e\in A(H_D)$ with source $u$ and target $v$, and let $F$ and $F'$ are the faces at the left-hand side and the right-hand side of $e$, respectively. Without loss of generality, suppose that the interior of $C$ is to the left-hand side of $Q$ (the other case is symmetric). We have four cases as follows.
\begin{itemize}
\item First, suppose that $e$ is in the exterior of $C$. Then, $f(F)^{-1}\cdot \phi(e)\cdot f(F')=\phi(e)$. By Definition \ref{def:innermostNonspiralBoringElimination}, $\psi(e)=\phi(e)$, and hence $f(F)^{-1}\cdot \phi(e)\cdot f(F')=\psi(e)$.

\item Second, suppose that $e\in A(C)\setminus A(Q)$. Then, $f(F)=1$ and $f(F')=t$ if $\dist_R(x,u)<\dist_R(x,v)$ (because in this case, the interior of $C$ is to the right-hand side of $e$), and $f(F)=t$ and $f(F')=1$ otherwise (because in this case, the interior of $C$ is to the left-hand side of $e$). Since $(\phi,\{\stitch_{\phi,v}\}|_{v\in V(H_D)})$ is shallow and the index $i$ of $e$ satisfies $|i|>|V(H_D)|-\distance(\phi,\{\stitch_{\phi,v}\}|_{v\in V(H_D)})$, we know that $\phi(e)=1$. Therefore, $f(F)^{-1}\cdot \phi(e)\cdot f(F')=t$ if $\dist_R(x,u)<\dist_R(x,v)$, and $f(F)^{-1}\cdot \phi(e)\cdot f(F')=t^{-1}$ otherwise. By Definition \ref{def:innermostNonspiralBoringElimination}, $\psi(e)=t$ if $\dist_R(x,u)<\dist_R(x,v)$, and $\psi(e)=t^{-1}$ otherwise. Hence, $f(F)^{-1}\cdot \phi(e)\cdot f(F')=\psi(e)$.

\item Third, suppose that $e\in A(Q)$. Then, $f(F)=t$ and $f(F')=1$ if $\dist_Q(x,u)<\dist_Q(x,v)$ (because in this case, the interior of $C$ is to the left-hand side of $e$), and $f(F)=1$ and $f(F')=t$ otherwise (because in this case, the interior of $C$ is to the right-hand side of $e$). By Definition \ref{def:wordExtraction} and Lemma \ref{lem:reconstructFlow}, we know that $\phi(e)=t^\epsilon$ where $\epsilon=1$ if $u$ is visited before $v$ when $Q$ is traversed from $x$ to $y$ (then, $\dist_Q(x,u)<\dist_Q(x,v)$), and $\epsilon=-1$ otherwise. Therefore, $f(F)^{-1}\cdot \phi(e)\cdot f(F')=t^{-1}\cdot t\cdot 1=1$ if $\dist_R(x,u)<\dist_R(x,v)$, and $f(F)^{-1}\cdot \phi(e)\cdot f(F')=1\cdot t^{-1}\cdot t = 1$ otherwise. By Definition \ref{def:innermostNonspiralBoringElimination}, $\psi(e)=1$, and hence $f(F)^{-1}\cdot \phi(e)\cdot f(F')=\psi(e)$.

\item Fourth, suppose that $e$ is in the strict interior of $C$. Then, $f(F)=f(F')=t$, and by Definition \ref{def:innermostNonspiralBoringElimination}, $\psi(e)=1$. Thus, to prove that $f(F)^{-1}\cdot \phi(e)\cdot f(F')=\psi(e)$, it suffices to show that $\phi(e)=1$. Since $Q$ is innermost, if $e$ does not belong to $A(R)$, then it is immediate that $\phi(e)=1$. Now, suppose that $e$ belongs to $A(R)$, which means that it is an arc parallel to some arc in $A(C)\cap A(R)$ between two vertices in $V_{=2}(R)$ (because $Q$ is a non-spiraling boring sequence). Recall that we indexed the arc copies of $e$, as well as the arc copies of any other arc in $A(R)$, by $e_{-|V(H_D)|},e_{-|V(H_D)|+1},\ldots,e_{-1},e_1,e_2,\ldots,e_{|V(H_D)|}$ so that they are ordered by their plane embedding, where $e_{-|V(H_D)|}$ and $e_{|V(H_D)|}$ are the outermost arcs, and so that the following condition holds: For every vertex $v\in V_{=2}(R)$, when the arcs incident to $v$ on $R$ (with all parallel copies) are enumerated in clockwise order starting at any arc, after an arc indexed $i\in\{-|V(H_D)|,|V(H_D)|\}$, we enumerated either a parallel arc or a not parallel arc indexed $i$. By Definition \ref{def:projectionNonspiralBoring}, this means that the index $i$ of $e$ must have absolute values larger than the index of the arcs in $\Project(Q)$. In particular, $|i|>|V(H_D)|-\distance(\phi,\{\stitch_{\phi,v}\}|_{v\in V(H_D)})$. Therefore, since $(\phi,\{\stitch_{\phi,v}\}|_{v\in V(H_D)})$ is shallow, we deduce that $\phi(e)=1$.
\end{itemize}
%Finally observe that $\psi$ is a well-behaved flow, since it is homologous to $\phi$. We apply Lemma~\ref{lem:pushedWeaklySimpleUsefulSubwalkModified} and a homologous flow $\psi'$ that is additionally weakly simplified, and identical to $\phi$ over $A(D)\setminus A(R)$. Then $\psi'$ is the required flow.
This completes the proof.
\end{proof}

Now, we turn to present the second step to complement Definition \ref{def:innermostNonspiralBoringElimination}, namely, we define the stitching-component of the elimination. Towards this, we give the following simple observation, which follows directly from Definitions \ref{def:walkWhoseSeqsArePaths} and \ref{def:shallow}.

\begin{observation}\label{obs:singleLetters}
Let $(D,S,T,g,k)$ be a nice instance of \dpdp. Let $R$ be a Steiner tree. Let $\phi: A(H_D)\rightarrow \RW(T)$ be a flow. Let $\{\stitch_{\phi,v}\}|_{v\in V(H_D)}$ be a stitching of $\phi$ such that $(\phi,\{\stitch_{\phi,v}\}|_{v\in V(H_D)})$ is shallow, non-cyclic and well-behaved. Then, for every arc $e\in A(H_D)$, it holds that $|\phi(e)|\leq 1$.
\end{observation}

Keeping Observation \ref{obs:singleLetters} in mind, the definition of the stitching-component is as follows. % (see Fig.~\hlg{FIG}).

\begin{definition}[{\bf Stitching-Component of Elimination of a Non-Spiral Boring Sequence}]\label{def:innermostNonspiralBoringEliminationStitching}
Let $(D,S,T,g,k)$ be a nice instance of \dpdp. Let $R$ be a Steiner tree. Let $\phi: A(H_D)\rightarrow \RW(T)$ be a flow. Let $\{\stitch_{\phi,v}\}|_{v\in V(H_D)}$ be a stitching of $\phi$ such that $(\phi,\{\stitch_{\phi,v}\}|_{v\in V(H_D)})$ is shallow, non-cyclic and well-behaved. Let $\cal W$ be the walk extraction of $(\phi,\{\stitch_{\phi,v}\}|_{v\in V(H_D)})$. Let $Q\in\Seq(W)$ for some $W\in{\cal W}$ be an innermost non-spiraling boring sequence. Let $\psi$ be the flow-component of the elimination of $Q$ in $(\phi,\{\stitch_{\phi,v}\}|_{v\in V(H_D)})$.
Then, the {\em stitching-component of the elimination of $Q$ in $(\phi,\{\stitch_{\phi,v}\}|_{v\in V(H_D)})$} is the collection $\{\stitch_{\psi,v}\}|_{v\in V(H_D)}$ of functions $\stitch_{\psi,v}: \Positions_v(\wl_{\psi})\rightarrow \Positions_v(\wl_{\psi})$ defined as follows.
\begin{itemize}
\item If $v\in V(Q)\setminus V(R)$, then $\Positions_v(\wl_{\psi})=\emptyset$, and hence $\stitch_{\psi,v}$ is defined. 
\item If $v\in V(H_D)\setminus V(\RB(Q))$, then define $\stitch_{\psi,v}=\stitch_{\phi,v}$.
\item If $v\in V(\RB(Q))\setminus V(Q)$, then $\Positions_v(\wl_{\psi})=\Positions_v(\wl_{\phi})\cup\{(e,1),(e',1)\}$ where $e$ and $e'$ are the two edges assigned non-empty words by $\psi$ but not by $\phi$. Then, define $\stitch_{\psi,v}$ as the extension of $\stitch_{\phi,v}$ that maps $(e,1)$ and $(e',1)$ to each other.
\item If $v\in V(Q)\cap V(R)$,\footnote{Note that $V(Q)\cap V(R)$ contain only the endpoints of $Q$.} then $\Positions_v(\wl_{\psi})=(\Positions_v(\wl_{\phi})\setminus\{(e,1)\})\cup\{(e',1)\}$ where $e$ is the edge incident to $v$ on $Q$ and $e'$ is the unique edge assigned a non-empty word by $\psi$ but not by $\phi$. Let $\widetilde{\stitch}_{\phi,v}$ be the restriction of $\stitch_{\phi,v}$ to $\Positions_v(\wl_{\phi})\setminus\{(e,1)\}$. Then, define $\stitch_{\psi,v}$ as the extension of $\widetilde{\stitch}_{\phi,v}$ that maps $\stitch_{\phi,v}(e,1)$ and $(e',1)$ to each other.
\end{itemize}
\end{definition}

We begin the analysis of the stitching-component by asserting that it is indeed a stitching of the flow-component.

\begin{observation}\label{obs:stitchingCompIsStitching}
Let $(D,S,T,g,k)$ be a nice instance of \dpdp. Let $R$ be a Steiner tree. Let $\phi: A(H_D)\rightarrow \RW(T)$ be a flow. Let $\{\stitch_{\phi,v}\}|_{v\in V(H_D)}$ be a stitching of $\phi$ such that $(\phi,\{\stitch_{\phi,v}\}|_{v\in V(H_D)})$ is shallow, non-cyclic and well-behaved. Let $\cal W$ be the walk extraction of $(\phi,\{\stitch_{\phi,v}\}|_{v\in V(H_D)})$. Let $Q\in\Seq(W)$ for some $W\in{\cal W}$ be an innermost non-spiraling boring sequence. Let $\psi$ and $\{\stitch_{\psi,v}\}|_{v\in V(H_D)}$ be the flow-component and the stitching-component, respectively, of the elimination of $Q$ in $(\phi,\{\stitch_{\phi,v}\}|_{v\in V(H_D)})$. Then, $\{\stitch_{\psi,v}\}|_{v\in V(H_D)}$ is a stitching of $\psi$.
\end{observation}

%\begin{proof}
%\hly{TODO}
%\end{proof}

Now, we identify the graphic representation of the elimination. The correctness of this observation is immediate from Definitions \ref{def:stitchingGraph} and \ref{def:innermostNonspiralBoringEliminationStitching}.

\begin{observation}\label{obs:eliminationGraphic}
Let $(D,S,T,g,k)$ be a nice instance of \dpdp. Let $R$ be a Steiner tree. Let $\phi: A(H_D)\rightarrow \RW(T)$ be a flow. Let $\{\stitch_{\phi,v}\}|_{v\in V(H_D)}$ be a stitching of $\phi$ such that $(\phi,\{\stitch_{\phi,v}\}|_{v\in V(H_D)})$ is shallow, non-cyclic and well-behaved. Let $\cal W$ be the walk extraction of $(\phi,\{\stitch_{\phi,v}\}|_{v\in V(H_D)})$. Let $Q\in\Seq(W)$ for some $W\in{\cal W}$ be an innermost non-spiraling boring sequence. Let $\psi$ and $\{\stitch_{\psi,v}\}|_{v\in V(H_D)}$ be the flow-component and the stitching-component, respectively, of the elimination of $Q$ in $(\phi,\{\stitch_{\phi,v}\}|_{v\in V(H_D)})$. Denote $\REP_{\phi}=\REP(\wl_{\phi},\{\stitch_{\phi,v}\}|_{v\in V(H_D)})$ and $\REP_{\psi}=\REP(\wl_{\psi},\{\stitch_{\psi,v}\}|_{v\in V(H_D)})$. Let ${\cal C}_\phi$ and ${\cal C}_\psi$ be the sets of connected components of $\REP_{\phi}$ and $\REP_{\psi}$, respectively. Then,
\begin{itemize}
\item There exist components $C_\phi\in{\cal C}_\phi$ and $C_\psi\in{\cal C}_\psi$ such that ${\cal C}_\phi\setminus\{C_\phi\}={\cal C}_\psi\setminus\{C_\psi\}$.
\item Let $x$ and $y$ be the endpoints of $Q$ where $x$ is visited first when $W$ is traversed from its endpoint $s\in S$ to its endpoint $g(s)\in T$.
Let $a_1,a_2,\ldots,a_p$ be the edges of $Q$ in the order in which they are visited when $W$ is traversed as before, and let $b_1,b_2,\ldots,b_q$ be the edges of $R$ assigned a letter by $\psi$ but not by $\phi$ in the order in which they are visited when the vertices of $\pathT_R(x,y)$ are traversed from $x$ to $y$. Then, $C_\psi$ equals $C_\phi$ where $(a_1,1)-(a_2,1)-\cdots-(a_p,1)$ is replaced by $(b_1,1)-(b_2,1)-\cdots-(b_q,1)$.
\end{itemize}
\end{observation}

By Definition \ref{def:walkExtraction} and Observation \ref{obs:eliminationGraphic}, we directly derive the following corollary, which asserts that the elimination is non-cyclic as well as identify its walk extraction.

\begin{corollary}\label{cor:eliminationWalkExtraction}
Let $(D,S,T,g,k)$ be a nice instance of \dpdp. Let $R$ be a Steiner tree. Let $\phi: A(H_D)\rightarrow \RW(T)$ be a flow. Let $\{\stitch_{\phi,v}\}|_{v\in V(H_D)}$ be a stitching of $\phi$ such that $(\phi,\{\stitch_{\phi,v}\}|_{v\in V(H_D)})$ is shallow, non-cyclic and well-behaved. Let $\cal W$ be the walk extraction of $(\phi,\{\stitch_{\phi,v}\}|_{v\in V(H_D)})$. Let $Q\in\Seq(W)$ for some $W\in{\cal W}$ be an innermost non-spiraling boring sequence. Let $\psi$ and $\{\stitch_{\psi,v}\}|_{v\in V(H_D)}$ be the flow-component and the stitching-component, respectively, of the elimination of $Q$ in $(\phi,\{\stitch_{\phi,v}\}|_{v\in V(H_D)})$. Then, $(\phi,\{\stitch_{\phi,v}\}|_{v\in V(H_D)})$ is non-cyclic. Furthermore, 
\begin{itemize}
\item There exist walks $W\phi\in{\cal W}_\phi$ and $W_\psi\in{\cal W}_\psi$ such that ${\cal W}_\phi\setminus\{W_\phi\}={\cal W}_\psi\setminus\{W_\psi\}$.
\item Let $x$ and $y$ be the endpoints of $Q$ where $x$ is visited first when $W$ is traversed from its endpoint $s\in S$ to its endpoint $g(s)\in T$.
Let $a_1,a_2,\ldots,a_p$ be the arcs of $Q$ in the order in which they are visited when $W$ is traversed as before, and let $b_1,b_2,\ldots,b_q$ be the arcs of $R$ assigned a letter by $\psi$ but not by $\phi$ in the order in which they are visited when $\pathT_R(x,y)$ is traversed from $x$ to $y$. Then, $W_\psi$ equals $W_\phi$ where (the subwalk that corresponds to the arc sequence) $a_1-a_2-\cdots-a_p$ is replaced by $b_1-b_2-\cdots-b_q$.
\end{itemize}
\end{corollary}

In turn, based on Corollary \ref{cor:eliminationWalkExtraction}, we assert that the elimination is shallow and well-behaved, and analyze its distance and weight.

\begin{lemma}\label{lem:eliminationProperties}
Let $(D,S,T,g,k)$ be a nice instance of \dpdp. Let $R$ be a Steiner tree. Let $\phi: A(H_D)\rightarrow \RW(T)$ be a flow. Let $\{\stitch_{\phi,v}\}|_{v\in V(H_D)}$ be a stitching of $\phi$ such that $(\phi,\{\stitch_{\phi,v}\}|_{v\in V(H_D)})$ is shallow, non-cyclic and well-behaved. Let $\cal W$ be the walk extraction of $(\phi,\{\stitch_{\phi,v}\}|_{v\in V(H_D)})$. Let $Q\in\Seq(W)$ for some $W\in{\cal W}$ be an innermost non-spiraling boring sequence. Let $\psi$ and $\{\stitch_{\psi,v}\}|_{v\in V(H_D)}$ be the flow-component and the stitching-component, respectively, of the elimination of $Q$ in $(\phi,\{\stitch_{\phi,v}\}|_{v\in V(H_D)})$. Then, $(\phi,\{\stitch_{\phi,v}\}|_{v\in V(H_D)})$ satisfies the following properties.
\begin{enumerate}
\item $\distance(\phi,\{\stitch_{\phi,v}\}|_{v\in V(H_D)})=\distance(\psi,\{\stitch_{\psi,v}\}|_{v\in V(H_D)})+1$.
\item $(\psi,\{\stitch_{\psi,v}\}|_{v\in V(H_D)})$ is shallow and well-behaved.
\item $\weight(\phi,\{\stitch_{\phi,v}\}|_{v\in V(H_D)})=\weight(\psi,\{\stitch_{\psi,v}\}|_{v\in V(H_D)})$.
\end{enumerate}
\end{lemma}

\begin{proof}
By Corollary \ref{cor:eliminationWalkExtraction}, the only difference between the sets of non-pushed sequences of the walk extractions of $(\phi,\{\stitch_{\phi,v}\}|_{v\in V(H_D)})$ and $(\psi,\{\stitch_{\psi,v}\}|_{v\in V(H_D)})$ is that $Q$ belongs to the first but not to the second. Therefore, $\distance(\phi,\{\stitch_{\phi,v}\}|_{v\in V(H_D)})=\distance(\psi,\{\stitch_{\psi,v}\}|_{v\in V(H_D)})$ $+1$, and since $(\phi,\{\stitch_{\phi,v}\}|_{v\in V(H_D)})$ is well-behaved, so is $(\psi,\{\stitch_{\psi,v}\}|_{v\in V(H_D)})$. In turn, because $\distance(\phi,\{\stitch_{\phi,v}\}|_{v\in V(H_D)})=\distance(\psi,\{\stitch_{\psi,v}\}|_{v\in V(H_D)})+1$ and $(\phi,\{\stitch_{\phi,v}\}|_{v\in V(H_D)})$ is shallow, to show that $(\psi,\{\stitch_{\psi,v}\}|_{v\in V(H_D)})$ is shallow, it suffices to show that the only arcs in $A(R)$ which are assigned letters by $\psi$ but not by $\phi$ have index of absolute value $|V(H_D)|-\distance(\phi,\{\stitch_{\phi,v}\}|_{v\in V(H_D)})+1$ (which equals $|V(H_D)|-\distance(\psi,\{\stitch_{\psi,v}\}|_{v\in V(H_D)})$), and that these arcs are assigned only a single letter. However, the correctness of this claim directly follows from Definition \ref{def:innermostNonspiralBoringElimination}.

To assert the third property, notice that by Corollary \ref{cor:eliminationWalkExtraction}, the only difference between the sets of useful subwalks of the walk extractions of $(\phi,\{\stitch_{\phi,v}\}|_{v\in V(H_D)})$ and $(\psi,\{\stitch_{\psi,v}\}|_{v\in V(H_D)})$ is in one useful subwalk consisting of only boring sequences, which in $(\phi,\{\stitch_{\phi,v}\}|_{v\in V(H_D)})$ contains $Q$ (and possibly other boring sequences), and in $(\psi,\{\stitch_{\psi,v}\}|_{v\in V(H_D)})$ contains (instead of $Q$) a subpath of $R$ that has no vertices in $V_{=1}(R)\cup V_{\geq 3}(R)$. Thus, $\weight(\phi,\{\stitch_{\phi,v}\}|_{v\in V(H_D)})=\weight(\psi,\{\stitch_{\psi,v}\}|_{v\in V(H_D)})$.
\end{proof}

We conclude and summarize the first phase in the following result.

\begin{lemma}\label{lem:phaseI}
Let $(D,S,T,g,k)$ be a nice instance of \dpdp. Let $R$ be a Steiner tree. Let $\phi: A(H_D)\rightarrow \RW(T)$ be a flow. Let $\{\stitch_{\phi,v}\}|_{v\in V(H_D)}$ be a stitching of $\phi$. Suppose that $(\phi,\{\stitch_{\phi,v}\}|_{v\in V(H_D)})$ is shallow, non-cyclic and well-behaved. Let $\Phi$ be the set of all pairs $(\widehat{\phi},\{\stitch_{\widehat{\phi},v}\}|_{v\in V(H_D)})$ of a flow $\widehat{\phi}$ and a stitching $\{\stitch_{\widehat{\phi},v}\}|_{v\in V(H_D)}$ of $\widehat{\phi}$ that satisfy the following properties:
\begin{itemize}
\item $\widehat{\phi}$ is homologous to $\phi$.
\item $(\widehat{\phi},\{\stitch_{\widehat{\phi},v}\}|_{v\in V(H_D)})$ is shallow, non-cyclic and well-behaved.
\item $\weight(\widehat{\phi},\{\stitch_{\widehat{\phi},v}\}|_{v\in V(H_D)})\leq \weight(\phi,\{\stitch_{\phi,v}\}|_{v\in V(H_D)})$.
\end{itemize}
Then, there exists $(\widehat{\phi},\{\stitch_{\widehat{\phi},v}\}|_{v\in V(H_D)})\in \Phi$ such that none of the walks in its walk extraction has a non-pushed non-spiraling boring sequence, and $\wh{\phi}$ is a weakly simplified flow.
\end{lemma}

\begin{proof}
Let $(\widehat{\phi},\{\stitch_{\widehat{\phi},v}\}|_{v\in V(H_D)})\in \Phi$ be a pair with minimum distance to $R$. We claim that none of the walks in its walk extraction $\cal W$ has a non-pushed non-spiraling boring sequence. Suppose, by way of contradiction, that this claim is false. Then, by Lemma \ref{lem:innermostNonspiralBoringExists},  there exists an innermost non-spiraling boring sequence $Q$ in $\Seq(W)$ for some walk $W\in{\cal W}$. Let $\psi$ and $\{\stitch_{\psi,v}\}|_{v\in V(H_D)}$ be the flow-component and the stitching-component, respectively, of the elimination of $Q$ in $(\widehat{\phi},\{\stitch_{\widehat{\phi},v}\}|_{v\in V(H_D)})$. From Lemma~\ref{lem:flowCompIsHomFlow} and Observation~\ref{obs:stitchingCompIsStitching}, $\psi$ is homologous to $\widehat{\phi}$ and hence to $\phi$ (since homology is a transitive relation), and $\{\stitch_{\psi,v}\}|_{v\in V(H_D)}$ is a stitching of $\psi$. Furthermore, by Corollary \ref{cor:eliminationWalkExtraction}, $(\psi,\{\stitch_{\psi,v}\}|_{v\in V(H_D)})$ is non-cyclic, and by Lemma \ref{lem:eliminationProperties}, it is also shallow and well-behaved. Additionally, by Lemma \ref{lem:eliminationProperties}, $\weight(\widehat{\phi},\{\stitch_{\widehat{\phi},v}\}|_{v\in V(H_D)})=\weight(\psi,\{\stitch_{\psi,v}\}|_{v\in V(H_D)})$. Because $\widehat{\phi}\in\Phi$, this implies that $\weight(\psi,\{\stitch_{\psi,v}\}|_{v\in V(H_D)})\leq \weight(\phi,\{\stitch_{\phi,v}\}|_{v\in V(H_D)})$. Thus, we conclude that $(\psi,\{\stitch_{\psi,v}\}|_{v\in V(H_D)})\in \Phi$. However, by Lemma \ref{lem:eliminationProperties}, $\distance(\widehat{\phi},\{\stitch_{\widehat{\phi},v}\}|_{v\in V(H_D)})>\distance(\psi,\{\stitch_{\psi,v}\}|_{v\in V(H_D)})$. This is a contradiction to the choice of $\widehat{\phi}$.
Finally, we apply Lemma~\ref{lem:pushedWeaklySimpleUsefulSubwalkModified} to ensure that $\wh{\phi}$ is also weakly simplified.
\end{proof}





\subsection{Phase II: Eliminating Non-Rollback Spirals}

We proceed pushing a flow onto a Steiner tree $R$ by canceling boring spirals with one another. Thus, Phases I and II together will eliminate all boring sequences. To this end, we need to identify which pair of boring spirals is to be pushed, based on Definition \ref{def:spiralPair}. Towards this, we first give the following definition concerning the endpoints of the two spirals in a spiral pair. We remind that a spiral pair $(Q,Q')$ is an ordered pair (in particular, $\RB(Q')$ contains $\RB(Q)$ in its interior).

\begin{definition}[{\bf Start, End, Extremes and Area of a Spiral Pair}]\label{def:spiralingPairArea}
Let $(D,S,T,g,k)$ be a nice instance of \dpdp. Let $R$ be a Steiner tree. Let $\phi: A(H_D)\rightarrow \RW(T)$ be a flow. Let $\{\stitch_{\phi,v}\}|_{v\in V(H_D)}$ be a stitching of $\phi$ such that $(\phi,\{\stitch_{\phi,v}\}|_{v\in V(H_D)})$ is non-cyclic and well-behaved. Let $\cal W$ be the walk extraction of $(\phi,\{\stitch_{\phi,v}\}|_{v\in V(H_D)})$. For a spiral pair $(Q,Q')$ (with respect to some group of spirals of some walk in $\cal W$), the {\em start} and {\em end} are the vertices among the endpoints of $Q$ and $Q'$ visited first and last when $W$ is traversed from its endpoint in $S$ to its endpoint in $T$, respectively. Moreover, the {\em extremes} of $(Q,Q')$ are the two endpoints $x$ and $y$ among the (at most four distinct) endpoints of $Q$ and $Q'$ of maximum distance on $R$. And its {\em area}, denoted by ${\sf area}(Q,Q')$, is the (unique) inner face of the subgraph of $H_D$ formed by $Q,Q'$ and $\pathT_R(x,y)$, that is bounded by both $Q$ and $Q'$.
\end{definition}

Now, we identified the promised pair. % (see Fig.~\hlg{FIG}).

\begin{definition}[{\bf Innermost Boring Spiral Pair}]\label{def:innermostBoringSpiralingPair}
Let $(D,S,T,g,k)$ be a nice instance of \dpdp. Let $R$ be a Steiner tree. Let $\phi: A(H_D)\rightarrow \RW(T)$ be a flow. Let $\{\stitch_{\phi,v}\}|_{v\in V(H_D)}$ be a stitching of $\phi$ such that $(\phi,\{\stitch_{\phi,v}\}|_{v\in V(H_D)})$ is non-cyclic and well-behaved. Let $\cal W$ be the walk extraction of $(\phi,\{\stitch_{\phi,v}\}|_{v\in V(H_D)})$. A spiral pair $(Q,Q')$ (with respect to some group of spirals of some walk in $\cal W$), is {\em innermost} if the strict interior of its area contains no arc that belongs to $(\bigcup_{W\in{\cal W}}A(W))\setminus A(R)$.
\end{definition}

We show that if there do not exist non-spiraling boring sequences in our collection, but there do exist boring spirals, then there exists at least one pair of boring spirals that is innermost.

\begin{lemma}\label{lem:innermostSpiralPairExists}
Let $(D,S,T,g,k)$ be a nice instance of \dpdp. Let $R$ be a Steiner tree. Let $\phi: A(H_D)\rightarrow \RW(T)$ be a weakly simplified flow. Let $\{\stitch_{\phi,v}\}|_{v\in V(H_D)}$ be a stitching of $\phi$ such that $(\phi,\{\stitch_{\phi,v}\}|_{v\in V(H_D)})$ is non-cyclic and well-behaved. Let $\cal W$ be the walk extraction of $(\phi,\{\stitch_{\phi,v}\}|_{v\in V(H_D)})$. If there do not exist non-pushed non-spiraling boring sequences in $\bigcup_{W\in{\cal W}}\Seq(W)$, and there exist spiraling boring sequences in $\bigcup_{W\in{\cal W}}\Seq(W)$, then there exists an innermost spiral pair $(Q,Q')$ with respect to some group of spirals of some walk in $W\in{\cal W}$. Furthermore, at most one useful subwalk of $W$ is between $Q$ and $Q'$ and it consists only of arcs in $A(R)$.
\end{lemma}

\begin{proof}
% These commands are defined only within this proof environment
\newcommand{\VR}{V_{=1}(R) \cup V_{\geq 3}(R)}
\newcommand{\W}{{\cal W}}
\renewcommand{\st}{\stitch}
\newcommand{\area}{{\sf area}}
%\hlb{TODO (PM): note that a spiral pair can have several forms dependent on where the endpoints of the two spirals are located relative to one another, and which (inner or outer) is the left-left one.}
Let $Q,Q'$ be a spiral pair. Then recall that by Definition~\ref{def:spiralPair}, there is a ring $\ring(S_u,S_v)$ corresponding to a pair of near vertices $u,v \in \VR$, such that $Q,Q'$ are contained in this ring (recall Definition~\ref{def:spiralPair} and Section~\ref{sec:winding}). Then it follows that both $\RB(Q)$ and $\RB(Q')$ contain the vertices of $\VR$ that lie in the interior of $S_u$ (Recall that the outer face lies in the unbounded region of $S_v$, and $S_u$ lies in the bounded region of $S_v$). Then by Observation~\ref{obs:SeqRBLaminar1}, we may assume that $\RB(Q') \cup I_{Q'} \subset \RB(Q) \cup I_Q$.
Now observe that the interior of $\area(Q,Q) = I_Q \setminus I_{Q'}$.
Let $W \in \cal W$ be the walk such that $Q,Q'$ are subwalks of $W$.
Suppose that, when traversing $W$, we first pass through $Q$ and then $Q'$. Let $x$ and $y$ be the first vertex of $Q$ and the last vertex of $Q'$ respectively in the traversal of $W$. Note that $Q,Q'$ are interesting sequences of $W$, and let $\wh{Q}$ be the boring subwalk in $\Use(W)$ between them (if any). Observe that as $\phi$ has no non-pushed non-spiraling boring sequences, all arcs of $\wh{Q}$ lie in $A(R)$. Thus $\wh{Q} \in \RUse(W)$, and since $\phi$ is weakly simplified, we have that $\wh{Q}$ is actually a subpath of $\pathT_R(u,v)$. Then we can conclude that the subwalk of $\W$ from $x$ to $y$ is an (undirected) path in $D$. Consider $\pathT_R[x,y]$ and note that it is a subpath of $\pathT_R[u,v]$. Observe that $\pathT_R[x,y]$ and $W[x,y]$ define a closed loop in the plane along the edges of $D$.
Indeed, this closed loop is almost a cycle, except for repeated vertices and parallel arcs on $V(\wh{Q}) \cap V(\pathT_R[x,y])$.
Furthermore, the interior of this closed loop is exactly $\area(Q,Q')$.

Let us choose $Q,Q'$ such that $\area(Q,Q')$ contains the fewest vertices of $V(D)$. 
Then we argue that $Q,Q'$ is an innermost boring spiral pair. 
Suppose not.
And let there be an arc $e \in (\bigcup_{W\in{\cal W}}A(W))\setminus A(R)$ that is contained in $\area(Q,Q')$. The arc $e$ must lie on some non-pushed sequence $P$, and by the premise of the lemma $P$ is a spiral. Then by Observation~\ref{obs:SeqRBLaminar2}, $P$ is contained in $\RB(Q)$, since the arc $e$ is contained in $\RB(Q)$.
First suppose that $P$ is a subpath of some walk $W' \in \W$ which is different from the walk $W$. Then, as $\pathT_R[x,y]$ and $W[x,y]$, and $\phi$ is a well-behaved flow, i.e. $Q,Q'$ and $P$ are vertex disjoint except for the endpoints, the endpoints of the walk $W'$ lies outside $\area(Q,Q')$ and there are non-pushed non-spirals in $\bigcup_{W \in \W} \Use(W)$, we have the following.
There is a spiral $P'$ such that $P,P'$ form a spiral pair and $\area(P,P') \subset \area(Q,Q')$. This immediately leads to a contradiction to our choice of the spiral pair $Q,Q'$.
And in the case where $P$ is a subwalk of walk $W$ (the same as $Q$ and $Q'$), since ${\sf sign}(Q) \neq {\sf sign}(Q')$ (since they are a spiral pair), one of them, say $Q$, forms a spiral pair with $P$. Then once again we have a spiral pair $P,Q$ such that $\area(P,Q) \subset \area(Q,Q')$, which is a contradiction.
\end{proof}

Towards the definition of the elimination of the spiral pair we have just identified, we need the following definition.
%(see Fig.~\hlg{FIG, show several diff spiral pairs}). 

\begin{definition}[{\bf Projection of a Spiral Pair}]\label{def:projectionSpiralPair}
Let $(D,S,T,g,k)$ be a nice instance of \dpdp. Let $R$ be a Steiner tree. Let $\phi: A(H_D)\rightarrow \RW(T)$ be a flow. Let $\{\stitch_{\phi,v}\}|_{v\in V(H_D)}$ be a stitching of $\phi$ such that $(\phi,\{\stitch_{\phi,v}\}|_{v\in V(H_D)})$ is shallow, non-cyclic and well-behaved. Let $\cal W$ be the walk extraction of $(\phi,\{\stitch_{\phi,v}\}|_{v\in V(H_D)})$. Let $(Q,Q')$ be an innermost spiral pair (with respect to some group of spirals of some walk in $\cal W$) with start $x$ and end $y$. Let $\ring(S_u,S_v)$ be the ring that contains $Q$. Then, the {\em projection of $(Q,Q')$ with respect to $(\phi,\{\stitch_{\phi,v}\}|_{v\in V(H_D)})$}, denoted by $\Project(Q,Q')$, is the set of arcs in $\bigcup_{e\in A(\pathT_R(x,y))}\Parallel(e)$, with the index 
\[b\cdot(|V(H_D)|-\dist(\phi,\{\stitch_{\phi,v}\}|_{v\in V(H_D)})+1),\] where $b\in\{-1,1\}$ is defined as follows. 
\begin{itemize}
\item %Consider the edge $e$ incident to $x$ on $Q$. 
First, consider the case where $Q$ is positive.\footnote{In this case, $Q$ is traversed from the left of $\pathT_R(u,v)$ and $Q'$ is traversed towards the left of $\pathT_R(u,v)$ (see Definitions \ref{def:spiralSign} and \ref{def:spiralPair}).} In this case, if the indices of leftmost edges of $\pathT_R(u,v)$ (when oriented from $u$ to $v$) are negative (i.e.~$-|V(H)|$), then $b=-1$, and otherwise (i.e.~they are $|V(H)|$) $b=1$.
\item Second, consider the case where $Q$ is positive. In this case, if the indices of rightmost edges of $\pathT_R(u,v)$ are negative , then $b=-1$, and otherwise $b=1$.
\end{itemize}
\end{definition}

We now show how to eliminate the spiral pair. This will be done in two steps. In the first step, we define the flow that results from the elimination. %(see Fig.~\hlg{FIG, show several diff spiral pairs}). 
Here, the implicit assumption concerning the uniqueness of $\widehat{Q}$ in the first item is supported by Lemma \ref{lem:innermostSpiralPairExists}.

\begin{definition}[{\bf Flow-Component of Elimination of a Spiral Pair}]\label{def:innermostSpiralPairElimination}
Let $(D,S,T,g,k)$ be a nice instance of \dpdp. Let $R$ be a Steiner tree. Let $\phi: A(H_D)\rightarrow \RW(T)$ be a flow. Let $\{\stitch_{\phi,v}\}|_{v\in V(H_D)}$ be a stitching of $\phi$ such that $(\phi,\{\stitch_{\phi,v}\}|_{v\in V(H_D)})$ is shallow, non-cyclic and well-behaved. Let $\cal W$ be the walk extraction of $(\phi,\{\stitch_{\phi,v}\}|_{v\in V(H_D)})$. Let $(Q,Q')$ be an innermost spiral pair (with respect to some group of spirals of some walk in $\cal W$). The {\em flow-component of the elimination of $(Q,Q')$ in $(\phi,\{\stitch_{\phi,v}\}|_{v\in V(H_D)})$} is the function $\psi: A(D)\rightarrow \RW(T)$ defined as follows, where $\widehat{Q}$ is the unique useful subwalk (if one exists)\footnote{If $\widehat{Q}$ does not exist, we treat $A(\widehat{Q})$ as an empty set.} between $Q$ and~$Q'$.
\begin{itemize}
\item For every arc $e\in A(Q)\cup A(Q')\cup A(\widehat{Q})$, define $\psi(e)=1$.
\item For every arc $e\in A(H_D)\setminus (A(Q)\cup A(Q')\cup A(\widehat{Q})\cup \Project(Q))$, define $\psi(e)=\phi(e)$.
\item Let $x$ and $y$ be the start and end of $(Q,Q')$, respectively. Then, for every arc $e\in\Project(Q,Q')$ with source $u$ and target $v$,
	\begin{itemize}
	\item if $\dist_R(x,u)<\dist_R(x,v)$,\footnote{Note that we measure the distance as the length of the shortest {\em undirected} path in $R$ between the two specified vertices.} then $\psi(e)=t$, and
	\item otherwise, $\psi(e)=t^{-1}$.
\end{itemize}
\end{itemize}
\end{definition}

First, we assert that the flow-component in Definition \ref{def:innermostNonspiralBoringElimination} is a flow homologous to its origin. Towards this, in addition to Proposition \ref{prop:functionOnFlow}, we need the following definition that refines the notion of an area in Definition \ref{def:spiralingPairArea} (see Fig~\ref{fig:preciseArea}). 
%,illustrated in Fig.~\hlg{FIG}. %\hlr{Need to extend the notion of simplified for non-pushed flow so that any useful subwalk that has only pushed sequences should be a path?}

\begin{figure}
    \begin{center}
\includegraphics[scale=0.6]{preciseArea.pdf}
        \caption{Precise area of a spiral pair.}
        \label{fig:preciseArea}
    \end{center}
\end{figure}

\begin{definition}[{\bf Precise Area}]\label{def:preciseArea}
Let $(D,S,T,g,k)$ be a nice instance of \dpdp. Let $R$ be a Steiner tree. Let $\phi: A(H_D)\rightarrow \RW(T)$ be a weakly simplified flow. Let $\{\stitch_{\phi,v}\}|_{v\in V(H_D)}$ be a stitching of $\phi$ such that $(\phi,\{\stitch_{\phi,v}\}|_{v\in V(H_D)})$ is shallow, non-cyclic and well-behaved. Let $\cal W$ be the walk extraction of $(\phi,\{\stitch_{\phi,v}\}|_{v\in V(H_D)})$. Consider a spiral pair $(Q,Q')$ with respect to some group of spirals of some walk in $\cal W$. Let $\widehat{Q}$ be the unique useful subwalk (if one exists) between $Q$ and $Q'$, and note that it is a subpath of a maximal degree-2 path in $R$ (since $\phi$ is a weakly simplified flow and by Observation~\ref{obs:newWeaklySimplifiedMeaning}). Let $x$ and $y$ be the start and end, respectively, of $(Q,Q')$. Let $p$ be the (unique) index of the arcs in $\Project(Q,Q')$. Let $P$ be the subpath of $R$ with endpoints $x$ and $y$ that consists of the arcs in $\Project(Q,Q')$. The {\em precise area} of $(Q,Q')$ is the union of three sets of faces, ${\cal F}_{\mathrm{proj}},{\cal F}_{\mathrm{area}}$ and ${\cal F}_{\mathrm{betw}}$, defined as follows.
\begin{itemize}
\item The set ${\cal F}_{\mathrm{proj}}$ contains every face of $H_D$ that is bounded (on both sides) by arcs $e_i$ and $e_{i+1}$ that {\em (i)} are each parallel to at least one arc in 
$\Project(Q,Q')$
%${\cal F}_{\mathrm{proj}}$, 
and {\em (ii)} whose indices $i$ and $i+1$ have the same sign as $p$ and satisfy $\min\{|i|,|i+1|\}\geq |p|$.

\item The set ${\cal F}_{\mathrm{area}}$ contains every face of $H_D$ that belongs to the area of $(Q,Q')$ and which is not bounded only by arcs in $A(R)$.

%\item The set ${\cal F}_{\mathrm{betw}}$ is the union of two sets of faces, ${\cal F}^1_{\mathrm{betw}}$ and ${\cal F}^2_{\mathrm{betw}}$, defined as follows. Let $L$ denote the set of every arc $e_i$ on the subpath of $R$ between $x$ and $y$ whose index $i$ is at least as small if $p$ is positive, and at least as large if $p$ is negative, than the indices of all arcs in $A(\widehat{Q})$ parallel to $e_i$. Then, ${\cal F}^1_{\mathrm{betw}}$ contains every face of $H_D$ that is bounded (on both sides) by arcs in $L$. If ${\cal F}_{\mathrm{proj}}$ contains at least one face to the left of $P$ (when oriented from $x$ to $y$), then let $d$ be right, and else let $d$ be left. Now, consider the graph $G$ on the arc set of $\widehat{Q}$. Let $\widehat{\cal F}^2_{\mathrm{betw}}$ be the faces of $G$ that are always to on the $d$-side of $\widehat{Q}$ when it is oriented from $x$ to $y$. Then, ${\cal F}^2_{\mathrm{betw}}$ contains every face of $H_D$ that is contained in a face in $\widehat{\cal F}^2_{\mathrm{betw}}$.
\item The set ${\cal F}_{\mathrm{betw}}$ is defined as follows. 
Recall that $\phi$ is a weakly simplified flow, and hence $\wh{Q}$ is a path that is a subpath of a maximal degree-2 path in $R$ (by Observation~\ref{obs:newWeaklySimplifiedMeaning}).
Let $L$ denote the set of every arc $e_i$ on the subpath of $R$ between $x$ and $y$ whose index $i$ is at least as small if $p$ is positive, and at least as large if $p$ is negative, than the index of the arc in $A(\widehat{Q})$ parallel to $e_i$. Then, ${\cal F}_{\mathrm{betw}}$ contains every face of $H_D$ that is bounded (on both sides) by arcs in $L$.
\end{itemize}
\end{definition}

We have the following claim regarding the precise area.

\begin{lemma}\label{lem:preciseArea}
Let $(D,S,T,g,k)$ be a nice instance of \dpdp. Let $R$ be a Steiner tree. Let $\phi: A(H_D)\rightarrow \RW(T)$ be a weakly simplified flow. Let $\{\stitch_{\phi,v}\}|_{v\in V(H_D)}$ be a stitching of $\phi$ such that $(\phi,\{\stitch_{\phi,v}\}|_{v\in V(H_D)})$ is shallow, non-cyclic and well-behaved. Let $\cal W$ be the walk extraction of $(\phi,\{\stitch_{\phi,v}\}|_{v\in V(H_D)})$. Consider an innermost spiral pair $(Q,Q')$ with respect to some group of spirals of some walk in $\cal W$. Let $x$ and $y$ be the start and end, respectively, of $(Q,Q')$, and let ${\cal F}_{\mathrm{prec}}$ be the precise area of $(Q,Q')$. Let $\widehat{Q}$ be the unique useful subwalk (if one exists) between $Q$ and $Q'$. Then, the following properties are satisfied.
\begin{enumerate}
\item\label{item:preciseAreaNoInc} For each arc $e$ that is not incident to any face in ${\cal F}_{\mathrm{prec}}$, it holds that $e\notin \Project(Q,Q')\cup A(Q)\cup A(Q')\cup A(\widehat{Q})$.

\item\label{item:preciseAreaIncTwo} For each arc $e$ incident to two faces in ${\cal F}_{\mathrm{prec}}$, it holds that {\em (i)} $\phi(e)=1$, and {\em (ii)} $e\notin \Project(Q,Q')\cup A(Q)\cup A(Q')\cup A(\widehat{Q})$. 

\item\label{item:preciseAreaExhaust} For each arc $e$ incident to exactly one face in ${\cal F}_{\mathrm{prec}}$, it holds that $e\in \Project(Q,Q')\cup A(Q)\cup A(Q')\cup A(\widehat{Q})$.

\item\label{item:preciseAreaProj} For each arc $e\in \Project(Q,Q')$, it holds that $e$ is incident to exactly one face in ${\cal F}_{\mathrm{proj}}$. Moreover, consider the subpath $P$ of $R$ with endpoints $x$ and $y$ that consists of the arcs in $\Project(Q,Q')$. Then, when $P$ is oriented from $x$ to $y$, the faces that the arcs in $\Project(Q,Q')$ in are incident to are either always on the left or always on the right.\footnote{Note that here, we disregard the direction of the arcs, and define sides according to the traversal of $P$ from $x$ to $y$.}

\item\label{item:preciseAreaQ} For each arc $e\in A(Q)\cup A(Q')\cup A(\widehat{Q})$, it holds that $e$ is incident to exactly one face in ${\cal F}_{\mathrm{proj}}$. Moreover, consider the subpath $P$ of $R$ with endpoints $x$ and $y$ that consists of the arcs in $\Project(Q,Q')$, and the subwalk $W'$ of $W$ with endpoints $x$ and $y$ that consists of the arcs in $A(Q)\cup A(Q')\cup A(\widehat{Q})$. Then, 
\begin{enumerate}
\item if when $P$ is oriented from $x$ to $y$, the faces in ${\cal F}_{\rm prec}$ that the arcs in $\Project(Q,Q')$ are incident to are always on the left, then when $W'$ is oriented from $x$ to $y$, the faces in ${\cal F}_{\rm prec}$ that the arcs in $A(Q)\cup A(Q')\cup A(\widehat{Q})$ in are incident to are always on the right;
\item else, when $W'$ is oriented from $x$ to $y$, the faces that the arcs in $A(Q)\cup A(Q')\cup A(\widehat{Q})$ in are incident to are always on the left.
\end{enumerate}
\end{enumerate}
\end{lemma}

\begin{proof}
Let $p, P$, $L, d$ and $G$ be as in Definition \ref{def:preciseArea}. Without loss of generality, suppose that $p$ is positive and $d$ is right. Observe that the $Q \cup Q' \cup \wh{Q}$, together with the arcs in $\Project(Q,Q')$, forms an closed loop along the edges of $D$ in the plane.
Note that this closed loop, when traversed in a cycle, any repeated vertices lie in $V(\Project(Q,Q')) \cap V(P) \subseteq V(R)$.
Indeed, this closed loop is almost an undirected cycle in $D$, except for the repeated vertices from $V(R)$~\footnote{The vertices of $V(\Project(Q,Q')) \cap V(P) \subseteq V(R)$ are visited at most twice in a single traversal of this closed loop.}.
Furthermore, the set of faces in the interior of this closed loop is exactly the collection of faces ${\cal F}_{\rm prec}$.
Also note that the subwalk of $W$ from $x$ to $y$ is a path consisting of the arcs in $A(Q) \cup A(Q') \cup A(\wh{Q})$. Here we use the fact that $\phi$ is a weakly simplified flow. Hence $Q, Q', \wh{Q}$ are all simple paths in $D$.
We now show that each of the properties is satisfied.

\smallskip
\noindent{\bf Property \ref{item:preciseAreaNoInc}.} This property follows from Properties \ref{item:preciseAreaProj} and \ref{item:preciseAreaQ}, which will be proved below.

\medskip
\noindent{\bf Property \ref{item:preciseAreaIncTwo}.} The second part of this property follows from Properties \ref{item:preciseAreaProj} and \ref{item:preciseAreaQ} that will be proved below. For the first part, consider some arc $e\notin \Project(Q,Q')\cup A(Q)\cup A(Q')\cup A(\widehat{Q})$ incident to two faces in ${\cal F}_{\mathrm{prec}}$. If $e$ is contained in ${\cal }_{\rm prec}$,  $(Q,Q')$ and is not in $A(R)$, then the constraint $\phi(e)=1$ follows from the supposition that $(Q,Q')$ is innermost. Else, if $e$ is parallel to an arc in $\Project(Q,Q')$ and has larger index than $p$, then then the constraint $\phi(e)=1$ follows from the supposition that $(\phi,\{\stitch_{\phi,v}\}|_{v\in V(H_D)})$ is shallow. Otherwise, by the definition of ${\cal F}_{\mathrm{prec}}$, it follows that $e$ must be incident on both sides to faces in ${\cal F}_{\mathrm{betw}}$. Here we once again use the supposition that $(\phi,\{\stitch_{\phi,v}\}|_{v\in V(H_D)})$.

\medskip
\noindent{\bf Property \ref{item:preciseAreaExhaust}.} If an arc $e$ is incident to exactly one face in ${\cal F}_{\rm prec}$, then the other face that $e$ is incident to lies outside ${\cal F}_{\rm prec}$.
In other words, $e$ lies on the boundary of the union of the faces in ${\cal F}_{\rm prec}$. Hence it holds that $e\in \Project(Q,Q')\cup A(Q)\cup A(Q')\cup A(\widehat{Q})$.

\medskip
\noindent{\bf Property \ref{item:preciseAreaProj}.} The definition of immediately implies that each arc $e_i\in \Project(Q,Q')$ is incident to exactly one face in ${\cal F}_{\mathrm{proj}}$, which is the face bounded by $e_p$ and its parallel copy $e_{p+1}$ (using the assumption that $p$ is positive).
%, and no face in ${\cal F}_{\mathrm{prec}}$
Next, when we traverse from $x$ to $y$ using the arcs in $\Project(Q,Q')$ observe that these arcs have the same index $p$ in their respective group of parallel arcs (by definition). Hence the faces that these arcs are incident to are either all on the left, or all on the right of the respective arcs.

\medskip
\noindent{\bf Property \ref{item:preciseAreaQ}.}
We recall the closed loop in $D$ formed by the subwalk of $W$ between $x$ and $y$, and the arcs in $\Project(Q,Q')$.
Let $W[x,y]$ denote this subwalk of $W$.
The first part is immediately clear, since all such arcs lie on the boundary of this closed loop. For the second part, note that if we traverse $P$ from $x$ to $y$, then since $W[x,y]$ forms the opposite side of this closed loop, the claim follows.
\end{proof}

We are now ready to analyze the flow-component.

\begin{lemma}\label{lem:flowCompIsHomFlow2}
Let $(D,S,T,g,k)$ be a nice instance of \dpdp. Let $\phi: A(H_D)\rightarrow \RW(T)$ be a weakly simplified flow. Let $\{\stitch_{\phi,v}\}|_{v\in V(H_D)}$ be a stitching of $\phi$ such that $(\phi,\{\stitch_{\phi,v}\}|_{v\in V(H_D)})$ is shallow, non-cyclic and well-behaved. Let $\cal W$ be the walk extraction of $(\phi,\{\stitch_{\phi,v}\}|_{v\in V(H_D)})$. Let $(Q,Q')$ be an innermost spiral pair (with respect to some group of spirals of some walk $W\in{\cal W}$). Then, the flow-component $\psi$ of the elimination of $(Q,Q')$ in $(\phi,\{\stitch_{\phi,v}\}|_{v\in V(H_D)})$ is a weakly simplified flow homologous to $\phi$.
\end{lemma}

\begin{proof}
Let $\cal F$ be the set of faces of $H_D$. In light of Proposition \ref{prop:functionOnFlow}, to prove the lemma, it suffices to show that there exists a function $f: {\cal F}\rightarrow \RW(\Sigma)$ such that {\em (i)} $f(F)=1$ for the outer face $F$ of $H_D$, and {\em (ii)} for every arc $e\in A(H_D)$, it holds that $f(F)^{-1}\cdot \phi(e)\cdot f(F')=\psi(e)$ where $F$ and $F'$ are the faces at the left-hand side and the right-hand side of $e$, respectively. We define a function $f: {\cal F}\rightarrow \RW(\Sigma)$ as follows. Let ${\cal F}_{\mathrm{prec}}$ be the precise area of $(Q,Q')$, let $x$ and $y$ be its start and end, respectively, and let $t$ be the endpoint of $W$ in $T$. Let $P$ be the subpath of $R$ with endpoints $x$ and $y$ that consists of the arcs in $\Project(Q,Q')$. Then, 
\begin{itemize}
\item for every face $F\in{\cal F}_{\mathrm{prec}}$, define $f(F)=t$ if when $P$ is oriented from $x$ to $y$, the faces the arcs in $\Project(Q,Q')$ in are incident to are always on the right, and $f(F)=t^{-1}$ if when $P$ is oriented from $x$ to $y$, the faces the arcs in $\Project(Q,Q')$ in are incident to are always on the left (by Condition \ref{item:preciseAreaProj} in Lemma \ref{lem:preciseArea}, exactly one of these conditions is~satisfied);
\item for every face $F\in{\cal F}\setminus {\cal F}_{\mathrm{prec}}$, define $f(F)=1$.
\end{itemize}
Since the outer face of $D$ is incident to a terminal, Condition {\em (i)} is clearly satisfied. Now, we turn to verify that Condition {\em (ii)} is satisfied. To this end, consider some arc $e\in A(H_D)$ with source $u$ and target $v$, and let $F$ and $F'$ are the faces at the left-hand side and the right-hand side of $e$, respectively. Without loss of generality, suppose that when $P$ is oriented from $x$ to $y$, the faces that the arcs $\Project(Q,Q')$ in are incident to are always on the right (the other case is symmetric). Let $\widehat{Q}$ be the unique useful subwalk (if one exists) between $Q$ and $Q'$. We have four cases as follows.
\begin{itemize}
\item First, suppose that $e$ is in not incident to any face in ${\cal F}_{\mathrm{prec}}$. Then, $f(F)^{-1}\cdot \phi(e)\cdot f(F')=\phi(e)$. By Condition \ref{item:preciseAreaNoInc} in Lemma \ref{lem:preciseArea}, $e\notin \Project(Q,Q')\cup A(Q)\cup A(Q')\cup A(\widehat{Q})$. Therefore, by Definition \ref{def:innermostSpiralPairElimination}, $\psi(e)=\phi(e)$, and hence $f(F)^{-1}\cdot \phi(e)\cdot f(F')=\psi(e)$.

\item Second, suppose that $e$ is incident to two faces in ${\cal F}_{\mathrm{prec}}$. Then, $f(F)=f(F')=t$, and by Condition \ref{item:preciseAreaIncTwo} in Lemma \ref{lem:preciseArea}, $\phi(e)=1$. Thus, $f(F)^{-1}\cdot \phi(e)\cdot f(F')=\phi(e)$. By Condition \ref{item:preciseAreaNoInc} in Lemma \ref{lem:preciseArea}, $e\notin \Project(Q,Q')\cup A(Q)\cup A(Q')\cup A(\widehat{Q})$. Therefore, by Definition \ref{def:innermostSpiralPairElimination}, $\psi(e)=\phi(e)$. Thus, we have that $f(F)^{-1}\cdot \phi(e)\cdot f(F')=\psi(e)$.

\item Third, suppose that $e\in \Project(Q,Q')$. Recall that we assumed that when $P$ is oriented from $x$ to $y$, the faces that the arcs $\Project(Q,Q')$ in are incident to are either always on the right. Therefore, $f(F)=1$ and $f(F')=t$ if $\dist_R(x,u)<\dist_R(x,v)$, and $f(F)=t$ and $f(F')=1$ otherwise. Since $(\phi,\{\stitch_{\phi,v}\}|_{v\in V(H_D)})$ is shallow and the index $i$ of $e$ satisfies $|i|>|V(H_D)|-\distance(\phi,\{\stitch_{\phi,v}\}|_{v\in V(H_D)})$ (by Definition \ref{def:projectionSpiralPair}), we know that $\phi(e)=1$. Thus, $f(F)^{-1}\cdot \phi(e)\cdot f(F')=t$ if $\dist_R(x,u)<\dist_R(x,v)$, and $f(F)^{-1}\cdot \phi(e)\cdot f(F')=t^{-1}$ otherwise. However, by Definition \ref{def:innermostSpiralPairElimination}, this means that $f(F)^{-1}\cdot \phi(e)\cdot f(F')=\psi(e)$.

\item Fourth, suppose that $e\in A(Q)\cup A(Q')\cup A(\widehat{Q})$. By Definition \ref{def:innermostSpiralPairElimination}, $\psi(e)=1$. Let $W'$ be the subwalk of $W$ with endpoints $x$ and $y$ that consists of the arcs in $A(Q)\cup A(Q')\cup A(\widehat{Q})$. Then, by Condition \ref{item:preciseAreaQ} in Lemma \ref{lem:preciseArea}, $e$ is incident to exactly one face in ${\cal F}_{\mathrm{prec}}$, and when $W'$ is oriented from $x$ to $y$, this face is on the left. This means that $f(F)=t$ and $f(F')=1$ if $W'$ (oriented from $x$ to $y$) visits $u$ before $v$ when traversing $e$, and that $f(F)=1$ and $f(F')=t$ otherwise. In turn, we get that $f(F)^{-1}\cdot \phi(e)\cdot f(F')=t^{-1}\cdot\phi(e)$ and if $W'$ visits $u$ before $v$ when traversing $e$, and $f(F)^{-1}\cdot \phi(e)\cdot f(F')=\phi(e)\cdot t$ otherwise. By Definition \ref{def:wordExtraction} and Lemma \ref{lem:reconstructFlow}, we know that $\phi(e)=t^\epsilon$ where $\epsilon=1$ if $W'$ visits $u$ before $v$ when traversing $e$, and $\epsilon=-1$ otherwise. Therefore, $f(F)^{-1}\cdot \phi(e)\cdot f(F')$ is necessarily $1$, and hence equal to $\psi(e)$.
\end{itemize}
By Condition \ref{item:preciseAreaExhaust} in Lemma \ref{lem:preciseArea}, every arc incident to exactly one face in ${\cal F}_{\mathrm{prec}}$ belongs to $\Project(Q,Q')\cup A(Q)\cup A(Q')\cup A(\widehat{Q})$. Thus, the case analysis above is exhaustive. Finally, we apply Lemma~\ref{lem:pushedWeaklySimpleUsefulSubwalkModified} to convert $\psi$ to a weakly simplified flow, and the proof is complete.
\end{proof}

Keeping Observation \ref{obs:singleLetters} in mind, we turn to present the second step to complement Definition \ref{def:innermostSpiralPairElimination}, namely, we define the stitching-component of the elimination. % (see Fig.~\hlg{FIG}). 

\begin{definition}[{\bf Stitching-Component of Elimination of a Spiral Pair}]\label{def:innermostSpiralPairEliminationStitching}
Let $(D,S,T,g,k)$ be a nice instance of \dpdp. Let $R$ be a Steiner tree. Let $\phi: A(H_D)\rightarrow \RW(T)$ be a flow. Let $\{\stitch_{\phi,v}\}|_{v\in V(H_D)}$ be a stitching of $\phi$ such that $(\phi,\{\stitch_{\phi,v}\}|_{v\in V(H_D)})$ is shallow, non-cyclic and well-behaved. Let $\cal W$ be the walk extraction of $(\phi,\{\stitch_{\phi,v}\}|_{v\in V(H_D)})$. Let $(Q,Q')$ be an innermost spiral pair (with respect to some group of spirals of some walk in $\cal W$). Let $x$ and $y$ be the start and end of $(Q,Q')$, respectively. Let $\psi$ be the flow-component of the elimination of $(Q,Q')$ in $(\phi,\{\stitch_{\phi,v}\}|_{v\in V(H_D)})$. Let $\widehat{Q}$ be the unique useful subwalk (if one exists) between $Q$ and $Q'$.
Then, the {\em stitching-component of the elimination of $(Q,Q')$ in $(\phi,\{\stitch_{\phi,v}\}|_{v\in V(H_D)})$} is the collection $\{\stitch_{\psi,v}\}|_{v\in V(H_D)}$ of functions $\stitch_{\psi,v}: \Positions_v(\wl_{\psi})\rightarrow \Positions_v(\wl_{\psi})$ defined as follows.
\begin{enumerate}
\item If $v\in (V(Q)\cup V(Q'))\setminus V(R)$, then $\Positions_v(\wl_{\psi})=\emptyset$, and hence $\stitch_{\psi,v}$ is defined. 
\item If $v\in V(H_D)\setminus (V(Q)\cup V(Q')\cup V(\widehat{Q})\cup V(\pathT_R(x,y)))$, then define $\stitch_{\psi,v}=\stitch_{\phi,v}$.

\item If $v\in V(\widehat{Q})\setminus V(\pathT_R(x,y))$, then $\Positions_v(\wl_{\psi})=\Positions_v(\wl_{\phi})\setminus\{(e,1),(e',1)\}$ where $e$ and $e'$ are the two edges assigned non-empty words by $\phi$ but not by $\psi$. Then, define $\stitch_{\psi,v}$ as the restriction of $\stitch_{\phi,v}$ to $\Positions_v(\wl_{\phi})\setminus\{(e,1),(e',1)\}$.

\item If $v\in V(\pathT_R(x,y))\setminus V(\widehat{Q})$, then we have two cases.
	\begin{itemize}
	\item If $v\notin\{x,y\}$, then $\Positions_v(\wl_{\psi})=\Positions_v(\wl_{\phi})\cup\{(e,1),(e',1)\}$ where $e$ and $e'$ are the two edges assigned non-empty words by $\psi$ but not by $\phi$. Then, define $\stitch_{\psi,v}$ as the extension of $\stitch_{\phi,v}$ that maps $(e,1)$ and $(e',1)$ to each other.
	\item Else, $\Positions_v(\wl_{\psi})=(\Positions_v(\wl_{\phi})\setminus\{(e,1)\})\cup\{(e',1)\}$ where $e$ is the edge incident to $v$ on $Q$ and $e'$ is the edge assigned a non-empty word by $\psi$ but not by $\phi$. Let $\widetilde{\stitch}_{\phi,v}$ be the restriction of $\stitch_{\phi,v}$ to $\Positions_v(\wl_{\phi})\setminus\{(e,1)\}$. Then, define $\stitch_{\psi,v}$ as the extension of $\widetilde{\stitch}_{\phi,v}$ that maps $\stitch_{\phi,v}(e,1)$ and $(e',1)$ to each other.
	\end{itemize}

\item If $v\in V(\widehat{Q})\cap V(\pathT_R(x,y))$, then we have two cases.
	\begin{itemize}
	\item If $v\notin\{x,y\}$, then $\Positions_v(\wl_{\psi})=(\Positions_v(\wl_{\phi})\setminus\{(e,1),(e',1)\})\cup\{(\widehat{e},1),(\widehat{e'},1)\}$ where $e$ and $e'$ are the two edges assigned non-empty words by $\phi$ but not by $\psi$, and $\widehat{e}$ and $\widehat{e}'$ are the two edges assigned non-empty words by $\psi$ but not by $\phi$. Let $\widetilde{\stitch}_{\phi,v}$ be the restriction of $\stitch_{\phi,v}$ to $\Positions_v(\wl_{\phi})\setminus\{(e,1),(e',1)\}$. Then, define $\stitch_{\psi,v}$ as the extension of $\widetilde{\stitch}_{\phi,v}$ that maps $(\widehat{e},1)$ and $(\widehat{e}',1)$ to each other.
	\item Else, $\Positions_v(\wl_{\psi})=(\Positions_v(\wl_{\phi})\setminus\{(e,1),(\widehat{e},1),(\widehat{e}',1)\})\cup\{(e',1)\}$ where $e$ is the edge incident to $v$ on $Q$, $\widehat{e}$ and $\widehat{e}'$ are the other two edges assigned non-empty words by $\phi$ but not by $\psi$, and $e'$ is the edge assigned a non-empty word by $\psi$ but not by $\phi$. Let $\widetilde{\stitch}_{\phi,v}$ be the restriction of $\stitch_{\phi,v}$ to $\Positions_v(\wl_{\phi})\setminus\{(e,1),(\widehat{e},1),(\widehat{e}',1)\}$. Then, define $\stitch_{\psi,v}$ as the extension of $\widetilde{\stitch}_{\phi,v}$ that maps $\stitch_{\phi,v}(e,1)$ and $(e',1)$ to each other.
	\end{itemize}
\end{enumerate}
\end{definition}

We begin the analysis of the stitching-component by asserting that it is indeed a stitching of the flow-component.

\begin{observation}\label{obs:stitchingCompIsStitching2}
Let $(D,S,T,g,k)$ be a nice instance of \dpdp. Let $R$ be a Steiner tree. Let $\phi: A(H_D)\rightarrow \RW(T)$ be a flow. Let $\{\stitch_{\phi,v}\}|_{v\in V(H_D)}$ be a stitching of $\phi$ such that $(\phi,\{\stitch_{\phi,v}\}|_{v\in V(H_D)})$ is shallow, non-cyclic and well-behaved. Let $\cal W$ be the walk extraction of $(\phi,\{\stitch_{\phi,v}\}|_{v\in V(H_D)})$. Let $(Q,Q')$ be an innermost spiral pair (with respect to some group of spirals of some walk in $\cal W$). Let $\psi$ and $\{\stitch_{\psi,v}\}|_{v\in V(H_D)}$ be the flow-component and the stitching-component, respectively, of the elimination of $(Q,Q')$ in $(\phi,\{\stitch_{\phi,v}\}|_{v\in V(H_D)})$. Then, $\{\stitch_{\psi,v}\}|_{v\in V(H_D)}$ is a stitching of $\psi$.
\end{observation}

%\begin{proof}
%\hly{TODO}
%\end{proof}

Now, we identify the graphic representation of the elimination.

\begin{observation}\label{obs:eliminationGraphic2}
Let $(D,S,T,g,k)$ be a nice instance of \dpdp. Let $R$ be a Steiner tree. Let $\phi: A(H_D)\rightarrow \RW(T)$ be a flow. Let $\{\stitch_{\phi,v}\}|_{v\in V(H_D)}$ be a stitching of $\phi$ such that $(\phi,\{\stitch_{\phi,v}\}|_{v\in V(H_D)})$ is shallow, non-cyclic and well-behaved. Let $\cal W$ be the walk extraction of $(\phi,\{\stitch_{\phi,v}\}|_{v\in V(H_D)})$. Let $(Q,Q')$ be an innermost spiral pair (with respect to some group of spirals of some walk $W\in{\cal W}$). Let $\psi$ and $\{\stitch_{\psi,v}\}|_{v\in V(H_D)}$ be the flow-component and the stitching-component, respectively, of the elimination of $(Q,Q')$ in $(\phi,\{\stitch_{\phi,v}\}|_{v\in V(H_D)})$. Denote $\REP_{\phi}=\REP(\wl_{\phi},\{\stitch_{\phi,v}\}|_{v\in V(H_D)})$ and $\REP_{\psi}=\REP(\wl_{\psi},\{\stitch_{\psi,v}\}|_{v\in V(H_D)})$. Let ${\cal C}_\phi$ and ${\cal C}_\psi$ be the sets of connected components of $\REP_{\phi}$ and $\REP_{\psi}$, respectively. Then,
\begin{itemize}
\item There exist components $C_\phi\in{\cal C}_\phi$ and $C_\psi\in{\cal C}_\psi$ such that ${\cal C}_\phi\setminus\{C_\phi\}={\cal C}_\psi\setminus\{C_\psi\}$.
\item Let $x$ and $y$ be the start and end of $(Q,Q')$, respectively. Let $\widehat{Q}$ be the unique useful subwalk (if one exists) between $Q$ and $Q'$. Let $a_1,a_2,\ldots,a_p$ be the edges of the subwalk of $W$ consisting of $Q,\widehat{Q}$ and $Q$ in the order they are visited when this subwalk is traversed from $x$ to $y$. Additionally, let $b_1,b_2,\ldots,b_q$ be the edges of $R$ assigned a letter by $\psi$ but not by $\phi$ in the order in which they are visited when $\pathT_R(x,y)$ is traversed from $x$ to $y$. Then, $C_\psi$ equals $C_\phi$ where $(a_1,1)-(a_2,1)-\cdots-(a_p,1)$ is replaced by $(b_1,1)-(b_2,1)-\cdots-(b_q,1)$.
\end{itemize}
\end{observation}

By Definition \ref{def:walkExtraction} and Observation \ref{obs:eliminationGraphic2}, we directly derive the following corollary, which asserts that the elimination is non-cyclic as well as identify its walk extraction.

\begin{corollary}\label{cor:eliminationWalkExtraction2}
Let $(D,S,T,g,k)$ be a nice instance of \dpdp. Let $R$ be a Steiner tree. Let $\phi: A(H_D)\rightarrow \RW(T)$ be a flow. Let $\{\stitch_{\phi,v}\}|_{v\in V(H_D)}$ be a stitching of $\phi$ such that $(\phi,\{\stitch_{\phi,v}\}|_{v\in V(H_D)})$ is shallow, non-cyclic and well-behaved. Let $\cal W$ be the walk extraction of $(\phi,\{\stitch_{\phi,v}\}|_{v\in V(H_D)})$. Let $(Q,Q')$ be an innermost spiral pair (with respect to some group of spirals of some walk $W\in{\cal W}$). Let $\psi$ and $\{\stitch_{\psi,v}\}|_{v\in V(H_D)}$ be the flow-component and the stitching-component, respectively, of the elimination of $(Q,Q')$ in $(\phi,\{\stitch_{\phi,v}\}|_{v\in V(H_D)})$. Then, $(\phi,\{\stitch_{\phi,v}\}|_{v\in V(H_D)})$ is non-cyclic. Furthermore, 
\begin{itemize}
\item There exist walks $W\phi\in{\cal W}_\phi$ and $W_\psi\in{\cal W}_\psi$ such that ${\cal W}_\phi\setminus\{W_\phi\}={\cal W}_\psi\setminus\{W_\psi\}$.
\item Let $x$ and $y$ be the start and end of $(Q,Q')$, respectively. Let $\widehat{Q}$ be the unique useful subwalk (if one exists) between $Q$ and $Q'$. Let $a_1,a_2,\ldots,a_p$ be the edges of the subwalk of $W$ consisting of $Q,\widehat{Q}$ and $Q$ in the order they are visited when this subwalk is traversed from $x$ to $y$. Additionally, let $b_1,b_2,\ldots,b_q$ be the edges of $R$ assigned a letter by $\psi$ but not by $\phi$ in the order in which they are visited when $\pathT_R(x,y)$ is traversed from $x$ to $y$. Then, $W_\psi$ equals $W_\phi$ where (the subwalk that corresponds to the arc sequence) $a_1-a_2-\cdots-a_p$ is replaced by $b_1-b_2-\cdots-b_q$.
\end{itemize}
\end{corollary}

In turn, based on Corollary \ref{cor:eliminationWalkExtraction2}, we assert that the elimination is shallow and well-behaved, and analyze its distance and weight.

\begin{lemma}\label{lem:eliminationProperties2}
Let $(D,S,T,g,k)$ be a nice instance of \dpdp. Let $R$ be a Steiner tree. Let $\phi: A(H_D)\rightarrow \RW(T)$ be a flow. Let $\{\stitch_{\phi,v}\}|_{v\in V(H_D)}$ be a stitching of $\phi$ such that $(\phi,\{\stitch_{\phi,v}\}|_{v\in V(H_D)})$ is shallow, non-cyclic and well-behaved. Let $\cal W$ be the walk extraction of $(\phi,\{\stitch_{\phi,v}\}|_{v\in V(H_D)})$. Let $(Q,Q')$ be an innermost spiral pair (with respect to some group of spirals of some walk in $\cal W$). Let $\psi$ and $\{\stitch_{\psi,v}\}|_{v\in V(H_D)}$ be the flow-component and the stitching-component, respectively, of the elimination of $(Q,Q')$ in $(\phi,\{\stitch_{\phi,v}\}|_{v\in V(H_D)})$. Then, $(\phi,\{\stitch_{\phi,v}\}|_{v\in V(H_D)})$ satisfies the following properties.
\begin{enumerate}
\item $\distance(\phi,\{\stitch_{\phi,v}\}|_{v\in V(H_D)})=\distance(\psi,\{\stitch_{\psi,v}\}|_{v\in V(H_D)})+2$.
\item $(\psi,\{\stitch_{\psi,v}\}|_{v\in V(H_D)})$ is shallow and well-behaved.
\item $\weight(\phi,\{\stitch_{\phi,v}\}|_{v\in V(H_D)})=\weight(\psi,\{\stitch_{\psi,v}\}|_{v\in V(H_D)})$.
\end{enumerate}
\end{lemma}

\begin{proof}
By Corollary \ref{cor:eliminationWalkExtraction2}, the only difference between the sets of non-pushed sequences of the walk extractions of $(\phi,\{\stitch_{\phi,v}\}|_{v\in V(H_D)})$ and $(\psi,\{\stitch_{\psi,v}\}|_{v\in V(H_D)})$ is that $Q$ and $Q'$ belong~to the first but not to the second. Thus, $\distance(\phi, \allowbreak \{\stitch_{\phi,v}\}|_{v\in V(H_D)})=\distance(\psi,\{\stitch_{\psi,v}\}|_{v\in V(H_D)})$ $+2$, and since $(\phi,\{\stitch_{\phi,v}\}|_{v\in V(H_D)})$ is well-behaved, so is $(\psi,\{\stitch_{\psi,v}\}|_{v\in V(H_D)})$. In turn, as $\distance(\phi,\{\stitch_{\phi,v}\}|_{v\in V(H_D)})=\distance(\psi,\{\stitch_{\psi,v}\}|_{v\in V(H_D)})+2$ and $(\phi,\{\stitch_{\phi,v}\}|_{v\in V(H_D)})$ is shallow, to show that $(\psi,\{\stitch_{\psi,v}\}|_{v\in V(H_D)})$ is shallow, it suffices to show that the only arcs in $A(R)$ which are assigned letters by $\psi$ but not by $\phi$ have index of absolute value $|V(H_D)|-\distance(\phi,\{\stitch_{\phi,v}\}|_{v\in V(H_D)})+1$ (which upper bounds $|V(H_D)|-\distance(\psi,\{\stitch_{\psi,v}\}|_{v\in V(H_D)})$), and that these arcs are assigned only a single letter. However, the correctness of this claim directly follows from Definition \ref{def:innermostSpiralPairElimination}.

To assert the third property, notice that by Corollary \ref{cor:eliminationWalkExtraction2}, the only difference between the sets of useful subwalks of the walk extractions of $(\phi,\{\stitch_{\phi,v}\}|_{v\in V(H_D)})$ and $(\psi,\{\stitch_{\psi,v}\}|_{v\in V(H_D)})$ is in one useful subwalk consisting of only boring sequences, which in $(\phi,\{\stitch_{\phi,v}\}|_{v\in V(H_D)})$ contains $Q$ and $Q'$ (and possibly other boring sequences), and in $(\psi,\{\stitch_{\psi,v}\}|_{v\in V(H_D)})$ these and the subwalk between them are replaced by a subpath of $R$ that has no vertices in $V_{=1}(R)\cup V_{\geq 3}(R)$. Thus, $\weight(\phi,\{\stitch_{\phi,v}\}|_{v\in V(H_D)})=\weight(\psi,\{\stitch_{\psi,v}\}|_{v\in V(H_D)})$.
\end{proof}

We conclude and summarize the second phase in the following result.

\begin{lemma}\label{lem:phaseII}
Let $(D,S,T,g,k)$ be a nice instance of \dpdp. Let $R$ be a Steiner tree. Let $\phi: A(H_D)\rightarrow \RW(T)$ be a flow. Let $\{\stitch_{\phi,v}\}|_{v\in V(H_D)}$ be a stitching of $\phi$. Suppose that $(\phi,\{\stitch_{\phi,v}\}|_{v\in V(H_D)})$ is shallow, non-cyclic and well-behaved. Let $\Phi$ be the set of all pairs $(\widehat{\phi},\{\stitch_{\widehat{\phi},v}\}|_{v\in V(H_D)})$ of a flow $\widehat{\phi}$ and a stitching $\{\stitch_{\widehat{\phi},v}\}|_{v\in V(H_D)}$ of $\widehat{\phi}$ that satisfy the following properties:
\begin{itemize}
\item $\widehat{\phi}$ is homologous to $\phi$.
\item $(\widehat{\phi},\{\stitch_{\widehat{\phi},v}\}|_{v\in V(H_D)})$ is shallow, non-cyclic and well-behaved.
\item $\weight(\widehat{\phi},\{\stitch_{\widehat{\phi},v}\}|_{v\in V(H_D)})\leq \weight(\phi,\{\stitch_{\phi,v}\}|_{v\in V(H_D)})$.
\end{itemize}
Then, there exists $(\widehat{\phi},\{\stitch_{\widehat{\phi},v}\}|_{v\in V(H_D)})\in \Phi$ such that none of the walks in its walk extraction has a non-pushed boring sequence, and $\wh{\phi}$ is a weakly simplified flow.
\end{lemma}

\begin{proof}
Let $(\widehat{\phi},\{\stitch_{\widehat{\phi},v}\}|_{v\in V(H_D)})\in \Phi$ be a pair with minimum distance to $R$. By Lemma \ref{lem:phaseI}, none of the walks in its walk extraction $\cal W$ has a non-pushed non-spiraling boring sequence.
Furthermore, $\wh{\phi}$ is a weakly simplified flow.
 We further claim that no walk in $\cal W$ has a spiraling boring sequence. Suppose, by way of contradiction, that this claim is false. Then, by Lemma \ref{lem:innermostSpiralPairExists},  there exists an innermost spiral pair $(Q,Q')$ (with respect to some group of spirals of some walk in $\cal W$). Let $\psi$ and $\{\stitch_{\psi,v}\}|_{v\in V(H_D)}$ be the flow-component and the stitching-component, respectively, of the elimination of $(Q,Q')$ in $(\widehat{\phi},\{\stitch_{\widehat{\phi},v}\}|_{v\in V(H_D)})$. From Lemma \ref{lem:flowCompIsHomFlow2} and Observation~\ref{obs:stitchingCompIsStitching2}, $\psi$ is homologous to $\widehat{\phi}$ and hence to $\phi$ (since homology is a transitive relation), and $\{\stitch_{\psi,v}\}|_{v\in V(H_D)}$ is a stitching of $\psi$. Furthermore, by Corollary \ref{cor:eliminationWalkExtraction2}, $(\psi,\{\stitch_{\psi,v}\}|_{v\in V(H_D)})$ is non-cyclic, and by Lemma \ref{lem:eliminationProperties2}, it is also shallow and well-behaved. Additionally, by Lemma \ref{lem:eliminationProperties2}, $\weight(\widehat{\phi},\{\stitch_{\widehat{\phi},v}\}|_{v\in V(H_D)})=\weight(\psi,\{\stitch_{\psi,v}\}|_{v\in V(H_D)})$. Because $\widehat{\phi}\in\Phi$, this implies that $\weight(\psi,\{\stitch_{\psi,v}\}|_{v\in V(H_D)})\leq \weight(\phi,\{\stitch_{\phi,v}\}|_{v\in V(H_D)})$. Thus, we conclude that $(\psi,\{\stitch_{\psi,v}\}|_{v\in V(H_D)})\in \Phi$. However, by Lemma \ref{lem:eliminationProperties2}, $\distance(\widehat{\phi},\{\stitch_{\widehat{\phi},v}\}|_{v\in V(H_D)})>\distance(\psi,\{\stitch_{\psi,v}\}|_{v\in V(H_D)})$. This is a contradiction to the choice of $\widehat{\phi}$.
\end{proof}






\subsection{Phase III: Eliminating Interesting Sequences}\label{sec:phaseIII}

Lastly, we finish pushing a flow onto a Steiner tree $R$ by pushing all interesting sequences. To this end, we need to identify which non-spiraling boring sequence is to be pushed. This is done in the following definition 
%(see Fig.~\hlg{FIG})
, based on the notion of $\RB(Q)$ in  Definition \ref{def:usefulSubwalkClosure}. 

\begin{definition}[{\bf Innermost Interesting Sequence}]\label{def:innermostInteresting}
Let $(D,S,T,g,k)$ be a nice instance of \dpdp. Let $R$ be a Steiner tree. Let $\phi: A(H_D)\rightarrow \RW(T)$ be a flow. Let $\{\stitch_{\phi,v}\}|_{v\in V(H_D)}$ be a stitching of $\phi$ such that $(\phi,\{\stitch_{\phi,v}\}|_{v\in V(H_D)})$ is non-cyclic and well-behaved. Let $\cal W$ be the walk extraction of $(\phi,\{\stitch_{\phi,v}\}|_{v\in V(H_D)})$. An interesting sequence $Q\in\Seq(W)$ for some $W\in{\cal W}$ is {\em innermost} if it is not pushed and the strict interior of $\RB(Q)$ contains no arc that belongs to $(\bigcup_{W\in{\cal W}}A(W))\setminus A(R)$.
\end{definition}

We show that if there do not exist boring sequences in our collection, but there do exist interesting sequences, then there exists at least one pair of boring spirals that is innermost.

\begin{lemma}\label{lem:innermostInterestingExists}
Let $(D,S,T,g,k)$ be a nice instance of \dpdp. Let $R$ be a Steiner tree. Let $\phi: A(H_D)\rightarrow \RW(T)$ be a flow. Let $\{\stitch_{\phi,v}\}|_{v\in V(H_D)}$ be a stitching of $\phi$ such that $(\phi,\{\stitch_{\phi,v}\}|_{v\in V(H_D)})$ is non-cyclic and well-behaved. Let $\cal W$ be the walk extraction of $(\phi,\{\stitch_{\phi,v}\}|_{v\in V(H_D)})$. If there do not exist non-pushed boring sequences in $\bigcup_{W\in{\cal W}}\Seq(W)$, and there exist non-pushed interesting sequences in $\bigcup_{W\in{\cal W}}\Seq(W)$, then there exists an innermost interesting sequence in $\bigcup_{W\in{\cal W}}\Seq(W)$.
\end{lemma}

\begin{proof}
As in the proof of Lemma~\ref{lem:innermostNonspiralBoringExists}, we choose a non-pushed interesting sequence $Q$ that minimizes the number of vertices of $V(D)$ that lie inside $\RB(Q)$. Then we can similarly argue that this is the required innermost sequence.
\end{proof}

Towards the definition of the elimination of the sequence we have just identified, we need the following definition.
% (see Fig.~\hlg{FIG}). 
Here, we remind that the parallel edges of $A(R)$ taken to construct $\RB(Q)$ are those indexed $1$.

\begin{definition}[{\bf Projection of Interesting Sequence}]\label{def:projectionInteresting}
Let $(D,S,T,g,k)$ be a nice instance of \dpdp. Let $R$ be a Steiner tree. Let $\phi: A(H_D)\rightarrow \RW(T)$ be a flow. Let $\{\stitch_{\phi,v}\}|_{v\in V(H_D)}$ be a stitching of $\phi$ such that $(\phi,\{\stitch_{\phi,v}\}|_{v\in V(H_D)})$ is shallow, non-cyclic and well-behaved. Let $\cal W$ be the walk extraction of $(\phi,\{\stitch_{\phi,v}\}|_{v\in V(H_D)})$. Let $Q\in\Seq(W)$ for some $W\in{\cal W}$ be an interesting sequence. Then, the {\em projection of $Q$ with respect to $(\phi,\{\stitch_{\phi,v}\}|_{v\in V(H_D)})$} is $\Project(Q)=\Project_{\mathrm{bou}}(Q)\cup\Project_{\mathrm{int}}(Q)$, where $\Project_{\mathrm{bou}}(Q)$ and $\Project_{\mathrm{int}}(Q)$ are defined as follows.
\begin{itemize}
\item First, $\Project_{\mathrm{bou}}(Q)$ is the set of arcs $e_i\in\bigcup_{e\in A(R)\cap \RB(Q)}\Parallel(e)$ with the index $i= b\cdot(|V(H_D)|-\dist(\phi,\{\stitch_{\phi,v}\}|_{v\in V(H_D)})+1)$, where $b\in\{-1,1\}$ is defined as follows.
\begin{itemize}
\item If the interior of $\RB(Q)$ contains edges in $A(R)$ indexed $-1$, then $b=-1$.
\item Otherwise, $b=1$.
\end{itemize}

\item Second, $\Project_{\mathrm{int}}(Q)$ is the set of arcs $e_i\in\bigcup_{e\in A(R)}\Parallel(e)$ that belong to the {\em strict} interior of $\RB(Q)$ with the index $i= b\cdot(|V(H_D)|-\dist(\phi,\{\stitch_{\phi,v}\}|_{v\in V(H_D)})+1)$ for both $b\in\{-1,1\}$. 
\end{itemize}
\end{definition}

Notice that, for a sequence $Q$ of a well-behaved walk, $\Project_{\mathrm{int}}(Q)$ can be empty, but because $Q$ has distinct endpoints, $\Project_{\mathrm{bou}}(Q)$ cannot be empty. Additionally, unless $\Project_{\mathrm{int}}(Q)$ is empty, the containment of an arc with one index implies the containment of the copy with the negated index, while in $\Project_{\mathrm{bou}}(Q)$, only one copy is present and it can contain (not parallel) arcs that have different indices (whose absolute value is the same). %, see Fig.~\hlg{FIG}.

%\begin{lemma}\label{lem:Project-bou} \hlr{incorrect}
%Let $(D,S,T,g,k)$ be a nice instance of \dpdp. Let $\phi: A(H_D)\rightarrow \RW(T)$ be a flow. Let $\{\stitch_{\phi,v}\}|_{v\in V(H_D)}$ be a stitching of $\phi$ such that $(\phi,\{\stitch_{\phi,v}\}|_{v\in V(H_D)})$ is shallow, non-cyclic and well-behaved. Let $\cal W$ be the walk extraction of $(\phi,\{\stitch_{\phi,v}\}|_{v\in V(H_D)})$. Let $Q\in\Seq(W)$ for some $W\in{\cal W}$ be an interesting sequence. Then, all arcs in $\Project_{\mathrm{bou}}(Q)$ have the same index.
%\end{lemma}

For an arc $e\in \Project_{\mathrm{int}}(Q)$, it is somewhat more involved to determine the sign of the letter which the flow-component assigns to $e$. In particular, we will rely on two notions, defined below. % (see Fig.~\hlg{FIG}).

\begin{definition}[{\bf $R$-Euler Circuit}]\label{def:eulerCirc}
Let $(D,S,T,g,k)$ be a nice instance of \dpdp. Let $R$ be a Steiner tree. The {\em $R$-Euler circuit} is the unique closed undirected walk $C$ in $R$ that visits every arc in $A(R)$ indexed $-1$ or $1$ exactly once and has the following property: For any traversal of $C$ (defined by any direction and start arc), for every arc $e_i$ which $C$ traverses from an endpoint $u$ to an endpoint $v\notin V_{=1}(R)$, the next arc that $C$ traverses is the unique arc $e'_j$ that is not $e_{-i}$ and is enumerated immediately after $e_i$ when the arcs incident to $v$ are ordered in either clockwise order or counter-clockwise order.
\end{definition}

Intuitively, an $R$-Euler circuit corresponds to the following operation: suppose that we ``cut open'' $R$ through its vertices and between every two arc copies indexed $1$ and $-1$; then, we obtain a cycle that can be viewed as the $R$-Euler circuit. Based on the notion of an $R$-Euler circuit, we further define the notion of a $Q$-Euler tour.

\begin{definition}[{\bf $Q$-Euler Tour}]\label{def:eulerTour}
Let $(D,S,T,g,k)$ be a nice instance of \dpdp. Let $R$ be a Steiner tree. Let $C$ be the $R$-Euler circuit. Let $\phi: A(H_D)\rightarrow \RW(T)$ be a flow. Let $\{\stitch_{\phi,v}\}|_{v\in V(H_D)}$ be a stitching of $\phi$ such that $(\phi,\{\stitch_{\phi,v}\}|_{v\in V(H_D)})$ is shallow, non-cyclic and well-behaved. Let $\cal W$ be the walk extraction of $(\phi,\{\stitch_{\phi,v}\}|_{v\in V(H_D)})$. Let $Q\in\Seq(W)$ for some $W\in{\cal W}$ be an innermost interesting sequence. Let $x$ and $y$ be the endpoints of $Q$ such that $x$ is visited before $y$ when $W$ is traversed from its endpoint $s\in S$ to its endpoint $g(s)\in T$. Then, the {\em $Q$-Euler tour} is the (unique) oriented subwalk of $C$ from $x$ to $y$ that visits every arc in $\{e_i\in A(C): \Project(Q)$ contains an arc parallel to $e_i$ and with the same sign$\}$ (not necessarily in the direction of the arc) exactly once.
\end{definition}

We now show how to eliminate the sequence. This will be done in two steps. In the first step, we define the flow that results from the elimination. % (see Fig.~\hlg{FIG}).

\begin{definition}[{\bf Flow-Component of Elimination of an Interesting Sequence}]\label{def:innermostInterestingElimination}
Let $(D,S,T,g,k)$ be a nice instance of \dpdp. Let $R$ be a Steiner tree. Let $\phi: A(H_D)\rightarrow \RW(T)$ be a flow. Let $\{\stitch_{\phi,v}\}|_{v\in V(H_D)}$ be a stitching of $\phi$ such that $(\phi,\{\stitch_{\phi,v}\}|_{v\in V(H_D)})$ is shallow, non-cyclic and well-behaved. Let $\cal W$ be the walk extraction of $(\phi,\{\stitch_{\phi,v}\}|_{v\in V(H_D)})$. Let $Q\in\Seq(W)$ for some $W\in{\cal W}$ be an innermost interesting sequence. Let $x$ and $y$ be the endpoints of $Q$ such that $x$ is visited before $y$ when $W$ is traversed from its endpoint $s\in S$ to its endpoint $g(s)\in T$. Then, the {\em flow-component of the elimination of $Q$ in $(\phi,\{\stitch_{\phi,v}\}|_{v\in V(H_D)})$} is the function $\psi: A(D)\rightarrow \RW(T)$ defined as~follows.
\begin{itemize}
\item For every arc $e\in A(Q)$, define $\psi(e)=1$.
\item For every arc $e\in A(H_D)\setminus (A(Q)\cup \Project(Q))$, define $\psi(e)=\phi(e)$.
%\item For every arc $e\in\Project_{\mathrm{bou}}(Q)$ with source $u$ and target $v$, if $\dist_R(x,u)<\dist_R(x,v)$, then $\psi(e)=t$, and otherwise, $\psi(e)=t^{-1}$.
\item Let $T$ be the $Q$-Euler tour. Then, for every arc $e_i\in\Project(Q)$ with source $u$ and target $v$, let  $e_j$ be the arc parallel to $e_i$ (or $e_i$ itself) where $j=1$ if $i\geq 1$ and $j=-1$ otherwise, and define $\psi(e_i)$ as follows.
\begin{itemize}
	\item If $T$ traverses $e_j$ from $u$ to $v$, then define $\psi(e_i)=t$.
	\item Otherwise ($T$ traverses $e_j$ from $v$ to $u$), define $\psi(e_i)=t^{-1}$.
\end{itemize}
\end{itemize}
\end{definition}

First, we assert that the flow-component in Definition \ref{def:innermostInterestingElimination} is a flow homologous to its origin.

\begin{lemma}\label{lem:flowCompIsHomFlow3}
Let $(D,S,T,g,k)$ be a nice instance of \dpdp. Let $R$ be a Steiner tree. Let $\phi: A(H_D)\rightarrow \RW(T)$ be a flow. Let $\{\stitch_{\phi,v}\}|_{v\in V(H_D)}$ be a stitching of $\phi$ such that $(\phi,\{\stitch_{\phi,v}\}|_{v\in V(H_D)})$ is shallow, non-cyclic and well-behaved. Let $\cal W$ be the walk extraction of $(\phi,\{\stitch_{\phi,v}\}|_{v\in V(H_D)})$. Let $Q\in\Seq(W)$ for some $W\in{\cal W}$ be an innermost interesting sequence. Then, the flow-component $\psi$ of the elimination of $Q$ in $(\phi,\{\stitch_{\phi,v}\}|_{v\in V(H_D)})$ is a flow homologous to $\phi$.
\end{lemma}

The proof of this lemma is similar to the proof of Lemma~\ref{lem:flowCompIsHomFlow}, but requires more arguments which rely on $Q$-Euler Tour.
%\begin{proof}
%\hly{TODO: requires more arguments than those in the proof in Phase 1; in particular, now arguments should rely on our def of $Q$-Euler tour.}
%\end{proof}

Keeping Observation \ref{obs:singleLetters} in mind, we turn to present the second step to complement Definition \ref{def:innermostInterestingElimination}, namely, we define the stitching-component of the elimination. 
%(see Fig.~\hlg{FIG}). 
For the validity of this definition, note that in any $Q$-Euler tour $T$, any vertex except for the endpoints is incident to an even number of edges, and each of the endpoints is incident to an odd number of edges; thus, the integer $p$ (in the definition) is an even number.

\begin{definition}[{\bf Stitching-Component of Elimination of an Interesting Sequence}]\label{def:innermostInterestingEliminationStitching}
Let $(D,S,T,g,k)$ be a nice instance of \dpdp. Let $\phi: A(H_D)\rightarrow \RW(T)$ be a flow. Let $\{\stitch_{\phi,v}\}|_{v\in V(H_D)}$ be a stitching of $\phi$ such that $(\phi,\{\stitch_{\phi,v}\}|_{v\in V(H_D)})$ is shallow, non-cyclic and well-behaved. Let $\cal W$ be the walk extraction of $(\phi,\{\stitch_{\phi,v}\}|_{v\in V(H_D)})$. Let $Q\in\Seq(W)$ for some $W\in{\cal W}$ be an innermost interesting sequence.  Let $T$ be the $Q$-Euler tour, and let $x$ and $y$ be the endpoints of $Q$. Let $\psi$ be the flow-component of the elimination of $Q$ in $(\phi,\{\stitch_{\phi,v}\}|_{v\in V(H_D)})$.
Then, the {\em stitching-component of the elimination of $Q$ in $(\phi,\{\stitch_{\phi,v}\}|_{v\in V(H_D)})$} is the collection $\{\stitch_{\psi,v}\}|_{v\in V(H_D)}$ of functions $\stitch_{\psi,v}: \Positions_v(\wl_{\psi})\rightarrow \Positions_v(\wl_{\psi})$ defined as follows.
\begin{itemize}
\item If $v\in V(Q)\setminus V(R)$, then $\Positions_v(\wl_{\psi})=\emptyset$, and hence $\stitch_{\psi,v}$ is defined. 
\item If $v\in V(H_D)\setminus (V(Q)\cup V(T))$, then define $\stitch_{\psi,v}=\stitch_{\phi,v}$.
\item If $v\in V(T)\setminus \{x,y\}$, then $\Positions_v(\wl_{\psi})=\Positions_v(\wl_{\phi})\cup\{(e,1): e\in A(T), e$ is incident to $v\}$. Then, $\stitch_{\psi,v}$ is the extension of $\stitch_{\phi,v}$ defined as follows. Let $a_1,a_2,\ldots,a_p$ be the arcs in $A(T)$ incident to $v$ enumerated in the order in which $T$ visits them.\footnote{Note that here, the subscript $i$ of $a_i$ does not refer to an index, and the arcs $a_i,a_j$ are not necessarily parallel.} Then, for each odd $i\in\{1,2,\ldots,p\}$, define $\stitch_{\psi,v}(a_i,1)=(a_{i+1},1)$, and for each even $i\in\{1,2,\ldots,p\}$, define $\stitch_{\psi,v}(a_i,1)=(a_{i-1},1)$.

\item If $v\in \{x,y\}$, then $\Positions_v(\wl_{\psi})=(\Positions_v(\wl_{\phi})\setminus\{(e,1)\})\cup\{(e',1): e'\in A(T), e'$ is incident to $v\}$ where $e$ is the edge incident to $v$ on $Q$. Let $\widetilde{\stitch}_{\phi,v}$ be the restriction of $\stitch_{\phi,v}$ to $\Positions_v(\wl_{\phi})\setminus\{(e,1)\}$. Then, $\stitch_{\psi,v}$ is the extension of $\widetilde{\stitch}_{\phi,v}$ defined as follows. Let $a_1,a_2,\ldots,a_{p+1}$ be the arcs in $A(T)$ incident to $v$ enumerated in the order in which $T$ visits them. Then, $\stitch_{\phi,v}$ maps $\stitch_{\phi,v}(e,1)$ and $(a_1,1)$ to each other. Additionally, for each even $i\in\{2,\ldots,p+1\}$, define $\stitch_{\psi,v}(a_i,1)=(a_{i+1},1)$, and for each odd $i\in\{2,\ldots,p+1\}$, define $\stitch_{\psi,v}(a_i,1)=(a_{i-1},1)$.
\end{itemize}
\end{definition}

We begin the analysis of the stitching-component by asserting that it is indeed a stitching of the flow-component.

\begin{observation}\label{obs:stitchingCompIsStitching3}
Let $(D,S,T,g,k)$ be a nice instance of \dpdp. Let $R$ be a Steiner tree. Let $\phi: A(H_D)\rightarrow \RW(T)$ be a flow. Let $\{\stitch_{\phi,v}\}|_{v\in V(H_D)}$ be a stitching of $\phi$ such that $(\phi,\{\stitch_{\phi,v}\}|_{v\in V(H_D)})$ is shallow, non-cyclic and well-behaved. Let $\cal W$ be the walk extraction of $(\phi,\{\stitch_{\phi,v}\}|_{v\in V(H_D)})$. Let $Q\in\Seq(W)$ for some $W\in{\cal W}$ be an innermost interesting sequence. Let $\psi$ and $\{\stitch_{\psi,v}\}|_{v\in V(H_D)}$ be the flow-component and the stitching-component, respectively, of the elimination of $Q$ in $(\phi,\{\stitch_{\phi,v}\}|_{v\in V(H_D)})$. Then, $\{\stitch_{\psi,v}\}|_{v\in V(H_D)}$ is a stitching of $\psi$.
\end{observation}

%\begin{proof}
%\hly{TODO}
%\end{proof}

Now, we identify the graphic representation of the elimination.

\begin{observation}\label{obs:eliminationGraphic3}
Let $(D,S,T,g,k)$ be a nice instance of \dpdp. Let $R$ be a Steiner tree. Let $\phi: A(H_D)\rightarrow \RW(T)$ be a flow. Let $\{\stitch_{\phi,v}\}|_{v\in V(H_D)}$ be a stitching of $\phi$ such that $(\phi,\{\stitch_{\phi,v}\}|_{v\in V(H_D)})$ is shallow, non-cyclic and well-behaved. Let $\cal W$ be the walk extraction of $(\phi,\{\stitch_{\phi,v}\}|_{v\in V(H_D)})$. Let $Q\in\Seq(W)$ for some $W\in{\cal W}$ be an innermost interesting sequence. Let $\psi$ and $\{\stitch_{\psi,v}\}|_{v\in V(H_D)}$ be the flow-component and the stitching-component, respectively, of the elimination of $Q$ in $(\phi,\{\stitch_{\phi,v}\}|_{v\in V(H_D)})$. Denote $\REP_{\phi}=\REP(\wl_{\phi},\{\stitch_{\phi,v}\}|_{v\in V(H_D)})$ and $\REP_{\psi}=\REP(\wl_{\psi},\{\stitch_{\psi,v}\}|_{v\in V(H_D)})$. Let ${\cal C}_\phi$ and ${\cal C}_\psi$ be the sets of connected components of $\REP_{\phi}$ and $\REP_{\psi}$, respectively. Then,
\begin{itemize}
\item There exist components $C_\phi\in{\cal C}_\phi$ and $C_\psi\in{\cal C}_\psi$ such that ${\cal C}_\phi\setminus\{C_\phi\}={\cal C}_\psi\setminus\{C_\psi\}$.
\item Let $T$ be the $Q$-Euler tour, and let $x$ and $y$ be the endpoints of $Q$ where $x$ is visited first when $W$ is traversed from its endpoint $s\in S$ to its endpoint $g(s)\in T$. Let $a_1,a_2,\ldots,a_p$ be the edges of $Q$ in the order in which they are visited when $W$ is traversed as before, and let $b_1,b_2,\ldots,b_q$ be the edges of $T$ when $T$ is traversed according to its orientation. Then, $C_\psi$ equals $C_\phi$ where $(a_1,1)-(a_2,1)-\cdots-(a_p,1)$ is replaced by $(b_1,1)-(b_2,1)-\cdots-(b_q,1)$.
\end{itemize}
\end{observation}

By Definition \ref{def:walkExtraction} and Observation \ref{obs:eliminationGraphic3}, we directly derive the following corollary, which asserts that the elimination is non-cyclic as well as identify its walk extraction.

\begin{corollary}\label{cor:eliminationWalkExtraction3}
Let $(D,S,T,g,k)$ be a nice instance of \dpdp. Let $R$ be a Steiner tree. Let $\phi: A(H_D)\rightarrow \RW(T)$ be a flow. Let $\{\stitch_{\phi,v}\}|_{v\in V(H_D)}$ be a stitching of $\phi$ such that $(\phi,\{\stitch_{\phi,v}\}|_{v\in V(H_D)})$ is shallow, non-cyclic and well-behaved. Let $\cal W$ be the walk extraction of $(\phi,\{\stitch_{\phi,v}\}|_{v\in V(H_D)})$. Let $Q\in\Seq(W)$ for some $W\in{\cal W}$ be an innermost interesting sequence. Let $\psi$ and $\{\stitch_{\psi,v}\}|_{v\in V(H_D)}$ be the flow-component and the stitching-component, respectively, of the elimination of $Q$ in $(\phi,\{\stitch_{\phi,v}\}|_{v\in V(H_D)})$. Then, $(\phi,\{\stitch_{\phi,v}\}|_{v\in V(H_D)})$ is non-cyclic. Furthermore, 
\begin{itemize}
\item There exist walks $W\phi\in{\cal W}_\phi$ and $W_\psi\in{\cal W}_\psi$ such that ${\cal W}_\phi\setminus\{W_\phi\}={\cal W}_\psi\setminus\{W_\psi\}$.
\item Let $T$ be the $Q$-Euler tour, and let $x$ and $y$ be the endpoints of $Q$ where $x$ is visited first when $W$ is traversed from its endpoint $s\in S$ to its endpoint $g(s)\in T$. Let $a_1,a_2,\ldots,a_p$ be the arcs of $Q$ in the order in which they are visited when $W$ is traversed as before, and let $b_1,b_2,\ldots,b_q$ be the edges of $T$ when $T$ is traversed according to its orientation. Then, $W_\psi$ equals $W_\phi$ where (the subwalk that corresponds to the arc sequence) $a_1-a_2-\cdots-a_p$ is replaced by $b_1-b_2-\cdots-b_q$.
\end{itemize}
\end{corollary}

In turn, based on Corollary \ref{cor:eliminationWalkExtraction2}, we assert that the elimination is shallow and well-behaved, and analyze its distance and weight.

\begin{lemma}\label{lem:eliminationProperties3}
Let $(D,S,T,g,k)$ be a nice instance of \dpdp. Let $R$ be a Steiner tree. Let $\phi: A(H_D)\rightarrow \RW(T)$ be a flow. Let $\{\stitch_{\phi,v}\}|_{v\in V(H_D)}$ be a stitching of $\phi$ such that $(\phi,\{\stitch_{\phi,v}\}|_{v\in V(H_D)})$ is shallow, non-cyclic and well-behaved. Let $\cal W$ be the walk extraction of $(\phi,\{\stitch_{\phi,v}\}|_{v\in V(H_D)})$. Let $Q\in\Seq(W)$ for some $W\in{\cal W}$ be an innermost interesting sequence. Let $\psi$ and $\{\stitch_{\psi,v}\}|_{v\in V(H_D)}$ be the flow-component and the stitching-component, respectively, of the elimination of $Q$ in $(\phi,\{\stitch_{\phi,v}\}|_{v\in V(H_D)})$. Then, $(\phi,\{\stitch_{\phi,v}\}|_{v\in V(H_D)})$ satisfies the following properties.
\begin{enumerate}
\item $\distance(\phi,\{\stitch_{\phi,v}\}|_{v\in V(H_D)})=\distance(\psi,\{\stitch_{\psi,v}\}|_{v\in V(H_D)})+1$.
\item $(\psi,\{\stitch_{\psi,v}\}|_{v\in V(H_D)})$ is shallow and well-behaved.
\item $\weight(\phi,\{\stitch_{\phi,v}\}|_{v\in V(H_D)})\geq \weight(\psi,\{\stitch_{\psi,v}\}|_{v\in V(H_D)})$.
\end{enumerate}
\end{lemma}

\begin{proof}
By Corollary \ref{cor:eliminationWalkExtraction3}, the only difference between the sets of non-pushed sequences of the walk extractions of $(\phi,\{\stitch_{\phi,v}\}|_{v\in V(H_D)})$ and $(\psi,\{\stitch_{\psi,v}\}|_{v\in V(H_D)})$ is that $Q$ belongs to the first but not to the second. Therefore, $\distance(\phi,\{\stitch_{\phi,v}\}|_{v\in V(H_D)})=\distance(\psi,\{\stitch_{\psi,v}\}|_{v\in V(H_D)})$ $+1$, and since $(\phi,\{\stitch_{\phi,v}\}|_{v\in V(H_D)})$ is well-behaved, so is $(\psi,\{\stitch_{\psi,v}\}|_{v\in V(H_D)})$. In turn, as $\distance(\phi,\{\stitch_{\phi,v}\}|_{v\in V(H_D)})=\distance(\psi,\{\stitch_{\psi,v}\}|_{v\in V(H_D)})+1$ and $(\phi,\{\stitch_{\phi,v}\}|_{v\in V(H_D)})$ is shallow, to show that $(\psi,\{\stitch_{\psi,v}\}|_{v\in V(H_D)})$ is shallow, it suffices to show that the only arcs in $A(R)$ which are assigned letters by $\psi$ but not by $\phi$ have index of absolute value $|V(H_D)|-\distance(\phi,\{\stitch_{\phi,v}\}|_{v\in V(H_D)})+1$ (which equals $|V(H_D)|-\distance(\psi,\{\stitch_{\psi,v}\}|_{v\in V(H_D)})$), and that these arcs are assigned only a single letter. However, the correctness of this claim directly follows from Definition \ref{def:innermostInterestingElimination}.

To assert the third property, notice that by Corollary \ref{cor:eliminationWalkExtraction3}, the only difference between the sets of useful subwalks of the walk extractions of $(\phi,\{\stitch_{\phi,v}\}|_{v\in V(H_D)})$ and $(\psi,\{\stitch_{\psi,v}\}|_{v\in V(H_D)})$ is as follows. The walk extraction of $(\phi,\{\stitch_{\phi,v}\}|_{v\in V(H_D)})$ has the non-pushed interesting useful subwalk $Q$, and two useful subwalks (which may or may not be interesting) $Q_1$ and $Q_2$ immediately before and after $Q$, respectively, in $W$.
Instead of $Q$, $(\psi,\{\stitch_{\psi,v}\}|_{v\in V(H_D)})$ has $x$ new pushed interesting useful subwalks, at most $x+1$ new pushed boring useful subwalks, and possibly $Q_1$ and $Q_2$ were elongated in case they were boring (in which case they stay boring), where $x$ is the number of arcs in $\Project(Q)$ that are incident to vertices in $V_{=1}(R)\cup V_{\geq 3}(R)$. By Observation \ref{obs:leaIntSteiner}, $|V_{=1}(R)\cup V_{\geq 3}(R)|\leq 4k-1$, and each one of these vertices can be incident to at most four arcs in $\Project(Q)$ (by Definition \ref{def:projectionInteresting}). Therefore, $2x+1<100k$. As the weight of each of the useful subwalks that belongs only to $(\psi,\{\stitch_{\psi,v}\}|_{v\in V(H_D)})$ is $1$,  while the weight of $Q$ is $100k$ (by Definition \ref{def:usefulSubwalkWeight}), we conclude that $\weight(\phi,\{\stitch_{\phi,v}\}|_{v\in V(H_D)})\geq\weight(\psi,\{\stitch_{\psi,v}\}|_{v\in V(H_D)})$.
\end{proof}

The conclusion of the third phase is given in Lemma \ref{lem:pusingFlowMain} in the next subsection.





\subsection{Existence of Non-Cyclic Pushed Flow with Low Weight}

We are now ready to fully push flows onto $R$.

\begin{lemma}\label{lem:pusingFlowMain}
Let $(D,S,T,g,k)$ be a nice instance of \dpdp. Let $R$ be a Steiner tree. Let $\phi: A(H_D)\rightarrow \RW(T)$ be a flow. Let $\{\stitch_{\phi,v}\}|_{v\in V(H_D)}$ be a stitching of $\phi$. Suppose that $(\phi,\{\stitch_{\phi,v}\}|_{v\in V(H_D)})$ is shallow, non-cyclic and well-behaved. Let $\Phi$ be the set of all pairs $(\widehat{\phi},\{\stitch_{\widehat{\phi},v}\}|_{v\in V(H_D)})$ of a flow $\widehat{\phi}$ and a stitching $\{\stitch_{\widehat{\phi},v}\}|_{v\in V(H_D)}$ of $\widehat{\phi}$ that satisfy the following properties:
\begin{itemize}
\item $\widehat{\phi}$ is homologous to $\phi$.
\item $(\widehat{\phi},\{\stitch_{\widehat{\phi},v}\}|_{v\in V(H_D)})$ is shallow and non-cyclic.
\item $\weight(\widehat{\phi},\{\stitch_{\widehat{\phi},v}\}|_{v\in V(H_D)})\leq \weight(\phi,\{\stitch_{\phi,v}\}|_{v\in V(H_D)})$.
\end{itemize}
Then, there exists $(\widehat{\phi},\{\stitch_{\widehat{\phi},v}\}|_{v\in V(H_D)})\in \Phi$ such that $\widehat{\phi}$ is pushed onto $R$.
\end{lemma}

\begin{proof}
Let $(\widehat{\phi},\{\stitch_{\widehat{\phi},v}\}|_{v\in V(H_D)})\in \Phi$ be a pair with minimum distance to $R$. We claim that none of the walks in its walk extraction $\cal W$ has a non-pushed sequence. Suppose, by way of contradiction, that this claim is false. By Lemma \ref{lem:phaseII}, none of the walks in $\cal W$ has a boring sequence.  Then, by Lemma \ref{lem:innermostInterestingExists}, there exists an innermost interesting sequence $Q$ in $\Seq(W)$ for some walk $W\in{\cal W}$. Let $\psi$ and $\{\stitch_{\psi,v}\}|_{v\in V(H_D)}$ be the flow-component and the stitching-component, respectively, of the elimination of $Q$ in $(\widehat{\phi},\{\stitch_{\widehat{\phi},v}\}|_{v\in V(H_D)})$. From Lemma \ref{lem:flowCompIsHomFlow3} and Observation~\ref{obs:stitchingCompIsStitching3}, $\psi$ is homologous to $\widehat{\phi}$ and hence to $\phi$ (since homology is a transitive relation), and $\{\stitch_{\psi,v}\}|_{v\in V(H_D)}$ is a stitching of $\psi$. Furthermore, by Corollary \ref{cor:eliminationWalkExtraction3}, $(\psi,\{\stitch_{\psi,v}\}|_{v\in V(H_D)})$ is non-cyclic, and by Lemma \ref{lem:eliminationProperties3}, it is also shallow and well-behaved. Additionally, by Lemma \ref{lem:eliminationProperties3}, $\weight(\widehat{\phi},\{\stitch_{\widehat{\phi},v}\}|_{v\in V(H_D)})\geq \weight(\psi,\{\stitch_{\psi,v}\}|_{v\in V(H_D)})$. Because $\widehat{\phi}\in\Phi$, this implies that $\weight(\psi,\{\stitch_{\psi,v}\}|_{v\in V(H_D)})\leq \weight(\phi,\{\stitch_{\phi,v}\}|_{v\in V(H_D)})$. Thus, we conclude that $(\psi,\{\stitch_{\psi,v}\}|_{v\in V(H_D)})\in \Phi$. However, by Lemma \ref{lem:eliminationProperties3}, $\distance(\widehat{\phi}, \allowbreak \{\stitch_{\widehat{\phi},v}\}|_{v\in V(H_D)})>\distance(\psi,\{\stitch_{\psi,v}\}|_{v\in V(H_D)})$. This is a contradiction to the choice of $\widehat{\phi}$. 
\end{proof}

\begin{figure}
    \begin{center}
        \includegraphics[scale=0.85]{FinalTreeFlow.pdf}
        \caption{The final pushed flow on the Steiner tree.}
        \label{fig:finalFlow}
    \end{center}
\end{figure}
Finally, we obtain the following result (see Fig~\ref{fig:finalFlow}).

\begin{lemma}\label{lem:pusingFlowMain2}
Let $(G,S',T',g',k)$ be a good \yes-instance of \pdp. Let $R'$ be a backbone Steiner tree. Let $(D,S,T,g,k)$ and $R$ be the orientations of $(G,S',T',g',k)$ and $R'$, respectively. Then, there exist a flow $\phi$ and a stitching $\{\stitch_{\phi,v}\}|_{v\in V(H_D)}$ of $\phi$ with the following properties, where $\cal W$ is the walk extraction of $(\phi,\{\stitch_{\phi,v}\}|_{v\in V(H_D)})$.
\begin{itemize}
\item $\phi$ is pushed onto $R$. Furthermore, $(\phi,\{\stitch_{\phi,v}\}|_{v\in V(H_D)})$ is simplified. %$\cal W$ is simplified.
\item $\phi$ is homologous to some flow associated with a solution of $(D,S,T,g,k)$.
\item $(\phi,\{\stitch_{\phi,v}\}|_{v\in V(H_D)})$ is shallow and non-cyclic.
\item $\sum_{W\in{\cal W}}|\Use(W)|\leq \alpha_{\mathrm{weight}}(k)$.
\end{itemize}
\end{lemma}

\begin{proof}
By Corollary \ref{cor:solFlowLowWeight}, $(D,S,T,g,k)$ admits a solution $\cal P$ such that $\weight({\cal P})\leq \alpha_{\mathrm{weight}}(k)$. Let $\psi: A(D)\rightarrow \RW(T)$ be the flow associated with $\cal P$, and $\{\stitch_{\psi,v}\}|_{v\in V(H_D)}$ be a stitching of $\psi$. By Lemma \ref{lem:solutionNonCyclic}, $(\phi,\{\stitch_{\phi,v}\}|_{v\in V(H_D)})$ is non-cyclic, and the walk extraction of $(\wl_{\phi},\{\stitch_{\phi,v}\}|_{v\in V(H_D)})$ is equal to $\cal P$. Thus, $(\phi,\{\stitch_{\phi,v}\}|_{v\in V(H_D)})$ is well-behaved, and $\weight(\psi)\leq \alpha_{\mathrm{weight}}(k)$. Without loss of generality, suppose that if some edge of $A(R)$ occurs in a path in $\cal P$, then this edge is of index $1$. As the paths in $\cal P$ are vertex disjoint, every vertex in $V(H_D)$ can belong to at most two sequences across al paths in $\cal P$, hence the distance between $(\phi,\{\stitch_{\phi,v}\}|_{v\in V(H_D)})$ and $R$ is upper bounded by $2|V(H_D)|-\ell$ where $\ell$ is the number of arcs of $A(R)$ occurs in a path in $\cal P$. From this, we deduce that $(\phi,\{\stitch_{\phi,v}\}|_{v\in V(H_D)})$ is shallow.

Notice that $\phi$ satisfies all suppositions in Lemma \ref{lem:pusingFlowMain}. Thus, by this lemma, there exist a flow $\widehat{\phi}$ and a stitching $\{\stitch_{\widehat{\phi},v}\}|_{v\in V(H_D)}$ of $\widehat{\phi}$ such that $\widehat{\phi}$ is homologous to $\phi$, $(\widehat{\phi},\{\stitch_{\widehat{\phi},v}\}|_{v\in V(H_D)})$ is shallow and non-cyclic, and $\weight(\widehat{\phi},\{\stitch_{\widehat{\phi},v}\}|_{v\in V(H_D)})\leq \weight(\phi,\{\stitch_{\phi,v}\}|_{v\in V(H_D)})$. As the number of useful subwalks (including repetitions) of a pair of a flow and a stitching is lower bounded by its weight, and $\weight(\psi)\leq \alpha_{\mathrm{weight}}(k)$, we derive that $\sum_{W\in{\cal W}_{\widehat{\phi}}}|\Use(W)|\leq \alpha_{\mathrm{weight}}(k)$ where ${\cal W}_{\widehat{\phi}}$ is the walk extraction of $(\widehat{\phi},\{\stitch_{\widehat{\phi},v}\}|_{v\in V(H_D)})$.

Lastly, notice that $\widehat{\phi}$ satisfies all suppositions in Lemma \ref{lem:pushedSimpleUsefulSubwalkModified}. Thus, by this lemma, there exist a pushed flow $\psi: A(H_D)\rightarrow \RW(T)$ and a stitching $\{\stitch_{\psi,v}\}|_{v\in V(H_D)}$ of $\psi$ such that {\em (i)} $\psi$ is homologous to $\widehat{\phi}$, {\em (ii)} $(\psi,\{\stitch_{\psi,v}\}|_{v\in V(H_D)})$ is shallow and non-cyclic, and {\em (iii)} $(\psi,\{\stitch_{\psi,v}\}|_{v\in V(H_D)})$ is simplified and its walk extraction ${\cal W}_{\psi}$ has the following property: $\sum_{W\in{\cal W}_{\psi}}|\Use({W})|\leq \sum_{W\in{\cal W}_{\widehat{\phi}}}|\Use(W)|$. As homology is a transitive relation and $\widehat{\phi}$ is homologous to $\phi$, we get that $\psi$ is homologous to a flow associated with a solution of $(D,S,T,g,k)$. As $\sum_{W\in{\cal W}_{\widehat{\phi}}}|\Use(W)|\leq \alpha_{\mathrm{weight}}(k)$, we also get that $\sum_{W\in{\cal W}_{\psi}}|\Use(W)|\leq \alpha_{\mathrm{weight}}(k)$. Thus, we conclude that $\psi$ has all properties in the statement of the lemma, hence the proof is complete.
\end{proof}

% remark that for a pushed flow $\phi$ and a stitching $\{\stitch_{\phi,v}\}|_{v\in V(H_D)}$ of $\phi$ such that $(\phi,\{\stitch_{\phi,v}\}|_{v\in V(H_D)})$ is non-cyclic, it necessarily holds that $(\phi,\{\stitch_{\phi,v}\}|_{v\in V(H_D)})$ is well-behaved as well, but we do not need to prove this claim as we do not need to use it. Moreover, we remark that the bound on the number of useful subwalks implies that the pushed flow assigns only short words. While it is easy to see this claim at this point, we do not show it now since it will be a consequence of arguments given later.


==> preamble.tex <==
\newcommand{\longversion}[1]{{#1}
\newcommand{\shortversion}[1]}

\usepackage[dvipsnames,svgnames,x11names]{xcolor}
\usepackage{amssymb,amsmath,mathrsfs}
\usepackage{soul}
\usepackage{mathtools}
\usepackage{framed}

\newcommand{\hlr}[1]{\sethlcolor{Salmon1}\hl{#1}\sethlcolor{yellow}} 
\newcommand{\hlg}[1]{\sethlcolor{PaleGreen2}\hl{#1}\sethlcolor{yellow}}
\newcommand{\hlb}[1]{\sethlcolor{SkyBlue1}\hl{#1}\sethlcolor{yellow}}
\newcommand{\hlo}[1]{\sethlcolor{Apricot}\hl{#1}\sethlcolor{yellow}}
\newcommand{\hly}[1]{\sethlcolor{Gold}\hl{#1}\sethlcolor{yellow}}

\usepackage{listings}
\usepackage{mathrsfs}
\usepackage[mathscr]{euscript}
\usepackage{amsfonts,amsthm,amsmath}
\usepackage{amstext}
\usepackage{graphicx,tikz}
\RequirePackage{fancyhdr}
\usepackage{boxedminipage}
\usepackage{todonotes}
%\usepackage[linesnumbered, boxed, algosection,noline]{algorithm2e}

\usepackage{graphics}
\usepackage{framed}
\usepackage{thm-restate}
\usepackage{thmtools}
\usepackage{enumerate}
\usepackage{float}
\usepackage{xspace}
%\usepackage{todonotes}

\newcommand{\OO}{\mathcal{O}}
\newcommand{\cO}{\mathcal{O}}

%\usepackage{vmargin}
%\setmarginsrb{1in}{1in}{1in}{1in}{0pt}{0pt}{0pt}{6mm}
\usepackage[margin=1in]{geometry}

\newcommand{\myparagraph}[1]{\smallskip\noindent{\textbf{\sffamily #1}}}

\newtheorem{theorem}{Theorem}[section]
\newtheorem{lemma}{Lemma}[section]
\newtheorem{claim}{Claim}[section]
\newtheorem{corollary}{Corollary}[section]
\newtheorem{definition}{Definition}[section]
\newtheorem{observation}{Observation}[section]
\newtheorem{proposition}{Proposition}[section]
\newtheorem{redrule}{Reduction Rule}[section]
\newtheorem{remark}{Remark}[section]
\newtheorem{reduction}{Reduction Rule}[section]
\newtheorem{conjecture}{Conjecture}[section]

\mathchardef\myhyphen="2D
 
\newcommand{\defparproblem}[4]{
\vspace{1mm}
\noindent\fbox{
  \begin{minipage}{0.96\textwidth}
  \begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}lr} #1  & {\bf{Parameter:}} #3 \\ \end{tabular*}
  {\bf{Input:}} #2  \\
  {\bf{Question:}} #4
  \end{minipage}
}\vspace{1mm}}

\newcommand{\defproblem}[3]{
\vspace{1mm}
\noindent\fbox{
  \begin{minipage}{0.96\textwidth}
  \begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}lr} #1 \\ \end{tabular*}
  {\bf{Input:}} #2  \\
  {\bf{Question:}} #3
  \end{minipage}
}\vspace{1mm}}

\usepackage{booktabs}
\usepackage[pdftex, plainpages = false, pdfpagelabels, 
                 %pdfpagelayout = useoutlines,
                 bookmarks=false,
                 bookmarksopen = true,
                 bookmarksnumbered = true,
                 breaklinks = true,
                 linktocpage,
                 pagebackref,
                 colorlinks = true,  % was true
                 linkcolor = blue,
                 urlcolor  = blue,
                 citecolor = red,
                 anchorcolor = green,
                 hyperindex = true,
                 hyperfigures
                 ]{hyperref}

% general
\newcommand{\yes}{\textsf{Yes}}
\newcommand{\no}{\textsf{No}}
\newcommand{\yesinstance}{\yes-instance}
\newcommand{\noinstance}{\no-instance}
\newcommand{\tw}{\mathtt{tw}}
\newcommand{\NP}{\textsf{NP}}
\newcommand{\coNP}{\textsf{co-NP}}
\newcommand{\FPT}{\textsf{FPT}}
\newcommand{\XP}{\text{XP}}
\newcommand{\WO}{\textsf{W[1]}}
\newcommand{\WOH}{\textsf{W[1]}-hard}
\newcommand{\WOC}{\textsf{W[1]}-complete}
\newcommand{\WTH}{\textsf{W[2]}-hard}
\newcommand{\WTC}{\textsf{W[2]}-complete}
\newcommand{\NPH}{\textsf{NP}-hard}
\newcommand{\NPC}{\textsf{NP}-complete}
\newcommand{\paraH}{\textsf{para-NP}-hard}
\newcommand{\ETH}{\textsf{ETH}}
\newcommand{\SETH}{\textsf{SETH}}
\newcommand{\nil}{\ensuremath{\mathtt{nil}}}
\newcommand{\dist}{\ensuremath{\mathsf{dist}}}
\newcommand{\flow}{\ensuremath{\mathsf{Flow}}}
\newcommand{\cupdot}{\mathbin{\mathaccent\cdot\cup}}

% specific
\newcommand{\pdp}{\textsf{Planar Disjoint Paths}}
\newcommand{\dpdp}{\textsf{Directed Planar Disjoint Paths}}
\newcommand{\deciPro}{\textsf{DecipherProcedure}}
\newcommand{\pdpAlg}{\textsf{PDPAlg}}
\newcommand{\deci}{\ensuremath{\mathsf{decipher}}}
\newcommand{\pathT}{\ensuremath{\mathsf{path}}}
\newcommand{\Sep}{\ensuremath{\mathsf{Sep}}}
\newcommand{\terminal}{\ensuremath{\mathsf{terminal}}}
\newcommand{\direction}{\ensuremath{\mathsf{direction}}}
\newcommand{\Enc}{\ensuremath{\mathsf{Enclose}}}
\newcommand{\word}{\ensuremath{\mathsf{word}}}
\newcommand{\rword}{\ensuremath{\mathsf{rword}}}
\newcommand{\unify}{\ensuremath{\mathsf{unify}}}
\newcommand{\ununify}{\ensuremath{\mathsf{ununify}}}
\newcommand{\sig}{\ensuremath{\mathsf{sign}}}
\newcommand{\weight}{\ensuremath{\mathsf{weight}}}
\newcommand{\distance}{\ensuremath{\mathsf{distance}}}
\newcommand{\Plunder}{\ensuremath{\mathsf{Plunder}}}
\newcommand{\RB}{\ensuremath{\mathsf{Bag}}}
\newcommand{\Seq}{\ensuremath{\mathsf{Seq}}}
\newcommand{\Seg}{\ensuremath{\mathsf{Seg}}}
\newcommand{\Use}{\ensuremath{\mathsf{Useful}}}
\newcommand{\Positions}{\ensuremath{\mathsf{Positions}}}
\newcommand{\wl}{\ensuremath{\mathsf{wl}}}
\newcommand{\stitch}{\ensuremath{\mathsf{stitch}}}
\newcommand{\component}{\ensuremath{\mathsf{component}}}
\newcommand{\conc}{\ensuremath{\mathsf{conc}}}
\newcommand{\pairing}{\ensuremath{\mathsf{pairing}}}
\newcommand{\stiPro}{\textsf{StitchProcedure}}
\newcommand{\walk}{\ensuremath{\mathsf{walk}}}
\newcommand{\template}{\ensuremath{\mathsf{template}}}
\newcommand{\trail}{\ensuremath{\mathsf{trail}}}
\newcommand{\REP}{\ensuremath{\mathsf{REP}}}
\newcommand{\ALL}{\ensuremath{\mathsf{ALL}}}
\newcommand{\ali}{\ensuremath{\mathsf{align}}}

%\newcommand{\R}{{\mathsf{RW}}}
\newcommand{\RW}{{\mathsf{RW}}}
\newcommand{\rdist}{{\mathsf{rdist}}}

% Weakly Useful subwalks
\newcommand{\RUse}{\ensuremath{\text{\sf R-Useful}}}

%ring-notes
\newcommand{\tin}{\mathrm{in}}
\newcommand{\tout}{\mathrm{out}}
%\newcommand{\crs}{\mathrm{cross}}
\newcommand{\crs}{\mathrm{traverse}}
\newcommand{\vis}{\mathrm{visitor}}
\newcommand{\Pp}{\mathcal{P}}
\newcommand{\Qq}{\mathcal{Q}}
\newcommand{\Cc}{\mathcal{C}}
\newcommand{\wh}[1]{\widehat{#1}}
\newcommand{\ring}{{\sf Ring}}
\newcommand{\lab}{{\sf label}}
\newcommand{\Rtwo}{{{\mathbb R}^2}}
\newcommand{\wn}{{\sf WindNum}}
\newcommand{\wnorig}{\overline{\sf WindNum}}
\newcommand{\order}{{\sf order}}
% 
% % crazy backreferencing
% %\documentclass{article}
% %\usepackage[colorlinks=true]{hyperref}
% %
% % START
% \usepackage{etoolbox,xstring,xspace}
% \makeatletter
% 
% \AtBeginDocument{%
%     \let\origref\ref
%     \renewcommand*\ref[1]{%
%         \origref{#1}\xlabel{#1}}
% }
% \newrobustcmd*\xlabel[1]{%
%     \ifcsdef{siteref@doc@#1}{}{\csgdef{siteref@doc@#1}{,}}%
%     \@bsphack%
%     \begingroup
%     \csxdef{siteref@doc@#1}{\csuse{siteref@doc@#1},\thepage}%
%     \protected@write\@auxout{}%
%     {\string\SiteRef{siteref@#1}{\csuse{siteref@doc@#1}}}%
%     \endgroup
%     \@esphack%
% }
% 
% \newrobustcmd*\SiteRef[2]{\csgdef{#1}{#2}}
% 
% \newrobustcmd*\xref[1]{%
%     \ifcsundef{siteref@#1}{%
%         \@latex@warning@no@line{Label `#1' not defined}
%     }{%
%         \begingroup
%         \StrGobbleLeft{\csuse{siteref@#1}}{2}[\@tempa]\relax%
%         \def\@tempb{}%
%         \@tempcnta=0\relax%
%         \@tempcntb=\@ne\relax%
%         \def\do##1{\advance\@tempcnta\@ne}%
%         \expandafter\docsvlist\expandafter{\@tempa}%
%         \def\do##1{%
%             \ifnum\@tempcntb=\@tempcnta\relax%
%             \hyperpage{##1}%
%             \else
%             \hyperpage{##1},%
%             \fi%
%             \advance\@tempcntb\@ne
%         }%
%         \expandafter\docsvlist\expandafter{\@tempa}\xspace%
%         \endgroup
%     }%
% }
% \makeatother
% \newcommand{\rlabel}[1]{\label{#1} {\rm({\footnotesize UsedOnPage: \xref{#1})}}}
%
% END
%\newcommand{\rlabel}[1]{\label{#1}}

%
% EXAMPLE
%\usepackage{lipsum}
%\begin{document}
%    \ref{tab:table}
%    \lipsum[1]
%    \begin{table}[!ht]
%        \begin{tabular}{ll}
%            \textbf{Name} & \textbf{Description} \\
%            Foo & bar \\
%            Foo & bar
%        \end{tabular}
%        \caption{Nice Table. Used on pages \xref{tab:table}.}
%        \label{tab:table}
%    \end{table}
%    
%    \lipsum
%    \ref{tab:table}
%\end{document}

